Misbehaviour Prediction for Autonomous Driving Systems

Deep Neural Networks (DNNs) are the core component of modern autonomous driving systems. To date, it is still unrealistic that a DNN will generalize correctly in all driving conditions. Current testing techniques consist of offline solutions that identify adversarial or corner cases for improving the training phase, and little has been done for enabling online healing of DNN-based vehicles. In this paper, we address the problem of estimating the confidence of DNNs in response to unexpected execution contexts with the purpose of predicting potential safety-critical misbehaviours such as out of bound episodes or collisions. Our approach SelfOracle is based on a novel concept of self-assessment oracle, which monitors the DNN confidence at runtime, to predict unsupported driving scenarios in advance. SelfOracle uses autoencoder and time-series-based anomaly detection to reconstruct the driving scenarios seen by the car, and determine the confidence boundary of normal/unsupported conditions. In our empirical assessment, we evaluated the effectiveness of different variants of SelfOracle at predicting injected anomalous driving contexts, using DNN models and simulation environment from Udacity. Results show that, overall, SelfOracle can predict 77% misbehaviours, up to 6 seconds in advance, outperforming the online input validation approach of DeepRoad by a factor almost equal to 3.

==> 6-discussion.tex <==
% !TEX root =  paper.tex
\section{Discussion}\label{sec:discussion} 

\begin{itemize}
\item What are the limits of our techniques, what mis-behaviour we were unable to detect? Was it the time to detection too short?
\end{itemize}


==> paper-anomaly-detection copy/0-abstract.tex <==
Deep Neural Networks (DNNs) are the core component of modern autonomous driving systems. 
To date, it is still unrealistic that a DNN will generalize correctly in all driving conditions. Current testing techniques consist of offline solutions that identify adversarial or corner cases for improving the training phase, and little has been done for enabling online healing of DNN-based vehicles. 

In this paper, we address the problem of estimating the confidence of  DNNs in response to unexpected execution contexts with the purpose of predicting potential safety-critical misbehaviours such as out of bound episodes or collisions. 
Our approach \tool is based on a novel concept of self-assessment oracle, which monitors  the DNN confidence at runtime, to predict unsupported driving scenarios in advance.
\tool uses autoencoder and time-series-based anomaly detection to reconstruct the driving scenarios seen by the car, and 
determine the confidence boundary of normal/unsupported conditions. 

In our empirical assessment, we evaluated the effectiveness of different  variants of \tool at predicting injected anomalous driving contexts, using DNN models and simulation environment from Udacity. Results show that, overall, \tool can predict 77\% misbehaviours, up to 6 seconds in advance, outperforming the online input validation approach of DeepRoad by a factor almost equal to 3.

%Autonomous driving systems are increasingly adopting deep neural networks (DNNs) for tasks, such as lane keeping or obstacle recognition, which require image processing for the generation of control signals for the car actuators. While DNN testing techniques can effectively discover adversarial or corner cases that are useful to improve the training phase, it is unrealistic to expect that a DNN will generalize correctly in all driving conditions. For this reason, a self-healing component takes control when the autopilot has low confidence. Depending on the level of autonomy, self-healing might involve the human driver or might be completely automated.
%
%In this paper, we propose a general approach for mis-behaviour prediction based on a self-assessment oracle that estimates the DNN confidence from time series analysis of the reconstruction errors \andrea{too many  buzzwords with no explanation within the same sentence: mis-behaviour + self-assessment oracle + confidence of a DNN + reconstruction error not clear. I'd cut the details on the Gamma, unnecessary in the abstract, and explain more on the problem of the paper}. We fit a Gamma probability distribution on such errors to determine the confidence threshold that activates self-healing. We have instantiated the approach in the tool \tool using different alternative reconstructors and we have evaluated its performance empirically on DNN models available for the Udacity autonomous car simulator. Results show that \tool can predict mis-behaviours with a tunable false alarm rate in nominal conditions and achieves promising mis-behaviour prediction performance\andrea{add the main results when complete}, outperforming the state-of-the-art approach of DeepRoad.

==> paper-anomaly-detection copy/1-introduction.tex <==
% !TEX root =  paper.tex
\section{Introduction}\label{sec:introduction}

\pagestyle{plain} % removes running headers

Self-driving cars are one of the emerging technologies nowadays, and possibly the standard way of transportation in the future. 
Such autonomous driving systems receive data from a multitude of sensors, and analyze them in real time using deep neural networks (DNNs) to determine the driving parameters for the actuators.
%DNN-based autonomous systems have shown great results in driving several hundreds of miles without any human intervention when a large amount of data is available~\cite{Cerf:2018:CSC:3181977.3177753,10-million-miles}.

%\head{How testing is performed}
To test such complex software systems, companies perform a limited number of expensive in-field tests, driving a car on real world streets, or within closed-course testing facilities~\cite{Cerf:2018:CSC:3181977.3177753}. This provides detailed sensor data of the vehicle that are recorded, played back, and recreated within a simulator to obtain comprehensive test scenarios.
Simulation-based test scenarios allow re-testing new autopilot releases on a large numbers of nominal conditions, as well as challenging (e.g., adverse weather) and dangerous circumstances (e.g., a pedestrian suddenly crossing the road), at a low cost~\cite{Cerf:2018:CSC:3181977.3177753}.

%include real driving situations from everyday nominal conditions, as well as challenging (e.g., adverse weather) and dangerous circumstances (e.g., a pedestrian suddenly crossing the drivable portion of the road), and allow re-testing of new autopilot releases on a large numbers of scenarios, which would be impossible to perform on-road
%As in classical regression testing, simulators allow for re-testing of new autopilot releases on a large numbers of scenarios, which would be impossible to perform on-road~\cite{Cerf:2018:CSC:3181977.3177753}.

%\head{Problem definition} 
%Despite the current efforts, testing autonomous vehicles is still considered one of the hardest engineering challenges~\cite{uber-cbs-article}. 
The potentially unlimited number of testable driving scenarios, combined with the lack of human interpretability of the internal functioning of DNNs~\cite{AlvarezMelisJ18}, makes it difficult to predict the vehicle's (mis-)behaviour with respect to unforeseen edge-case scenarios. 
Misbehaviours span a wide range of situations, associated with different degrees of severity, from cases where the car does not drive smoothly (e.g., excessively high derivative of the steering angle over time), to safety-critical failures and casualties~\cite{tesla-accident-1,tesla-accident-2,tesla-accident-3,tesla-accident-4}.
In this respect, promptly detecting unexpected, untested behaviours is of paramount importance, so as to make sure that human-driven or self-healing corrective actions take place to ensure safety.

In this paper, we tackle the \textit{self-assessment oracle problem} for autonomous driving system, i.e., the problem of monitoring the confidence level of a DNN-based autonomous driving system in order to timely predict the occurrence of future misbehaviours. 
The problem is critical because a failure in detecting an unexpected condition may have severe consequences (i.e., a fatal crash), whereas false alarms, even if not dangerous, may cause driver's discomfort and negatively affect the driving experience. Creating a self-assessment oracle that evaluates the confidence of a DNN \textit{at runtime}, and predicts whether the system is within a low-confidence zone, is a largely unexplored research problem.

Challenges arise because unexpected driving conditions are, by definition, unknown at training time, otherwise they would be used to train a better DNN~\cite{Campos:2016:EUO:2962863.2962870}. As a consequence, the problem being addressed belongs to the unsupervised class of data analysis,  %no data point in the training set is labelled as ``unexpected'', and the only available information is about the ``normal'' data points. 
and we have to infer the unexpected only by looking at the normal driving scenarios.
Moreover, the ensemble of possible misbehaviours for a DNN-based system is vast and necessarily domain-dependent, being associated with deviations from the functional requirements. 
%, which depend on the domain in which DNNs are used. 
%\andrea{kinda repeated from above}
%because misbehaviours are rare, so knowledge about them cannot be obtained from observations. 
%because the very definition of misbehaviour is domain-dependent: misbehaviours are associated with major deviations from the functional requirements, which depend on the domain in which DNNs are used. 
%
%Indeed, a major obstacle consists in the lack of labeled anomaly datasets for self-driving vehicles~\cite{Campos:2016:EUO:2962863.2962870}. 
%Though anomaly detection has been a widely studied problem, there is still a lack of commonly agreed upon benchmark datasets~\cite{}. 
%In some domains, it is sufficient to have tolerance levels, and any value outside the tolerance intervals is considered as an anomaly.
%Last, early and accurate confidence estimation for self-driving cars should take into account the temporal dimension, i.e., the entire time series of driving conditions. 
%\andrea{still looks a weak point to me}
%\andrea{If results show that single-based AD performs as good as LSTM, we should take care of this sentence}
%In fact, by observing a decreasing confidence trend over time we can anticipate a misbehaviour by predicting the future confidence values. At the same time, by observing an entire time window we can get rid of noisy, spiky values, where confidence falls below threshold for a very short time  
%\andrea{if results support us, we can make a nice claim here}
%Indeed, the temporal dimension is also worth considering, as the historical information about the car's (mis-)behaviour may signal a deviation from the expected behaviour.

%\head{Existing techniques} 
In recent years, researchers have proposed solutions for testing autonomous driving systems software~\cite{deepsafe,Gambi:2019:ATS:3293882.3330566,deepxplore,deeptest,deeproad,Abdessalem-ASE18-1,Abdessalem-ASE18-2,Abdessalem-ICSE18,deepsafe}. 
A number of approaches propose input generation techniques that produce corner/adversarial cases, used to improve the robustness of self-driving car modules by re-training~\cite{deepxplore,deeptest,deeproad,Kim:2019:GDL:3339505.3339634}. Other works target test case generation to expose faults for extreme conditions, such as the vehicle colliding with a pedestrian~\cite{Abdessalem-ICSE18}, or driving off the road~\cite{Gambi:2019:ATS:3293882.3330566}.
All these approaches concern \textit{offline} solutions for improving the robustness and reliability of DNNs, achieved by enhancing the training data and the autopilot module, which are extended to include underrepresented critical scenarios. 
%These solutions essentially exploit the well-known lack of robustness of DNNs to adversarial examples. 
%Thus, the main use-case of such studies concern identifying underrepresented critical scenarios \textit{offline} in the training data (e.g., snowy weather conditions), and provide means for a more focused training of autonomous driving systems. 
%Indeed, results from these papers have shown that such adversarial examples are easily avoided by retraining the DNN. 
To the best of our knowledge, no existing work is focused on online confidence estimation for self-driving vehicles with  
the aim of anticipating the occurrence of misbehaviours so as to enable self-healing procedures that can avoid future failures. 

%\andrea{This part cuts the flow, and creates overexpectations; I used it into the background section}
%In self-driving cars, depending on the level of autonomy the self-healing procedure might either involve the human driver or might be delegated to an automated system. At NHTSA Level 4 (High Automation)\footnote{https://www.nhtsa.gov/technology-innovation/automated-vehicles-safety}, the autopilot disengages in extreme (e.g., rainy/snowy) driving conditions and the human is requested to intervene. At Level 5 (Full Automation -- the highest NHTSA level), all functionalities are handled automatically, including safe disengagement: e.g., an automated disengagement module may safely park the car when misbehaviours or failures are detected (e.g., a flat wheel). At both top levels of autonomy, early and accurate misbehaviour prediction is an essential component of the overall driving system.

%and the applicability of input validation technique such as DeepXplore or DeepTest to this problem is quite limited. Indeed, it is likely impractical to \textit{early} detect anomalous behaviours only by considering individual inputs (i.e., an image). 
%
%Moreover, if the driving scenario is getting increasingly challenging (for instance, a snow storm approaching the vehicle), it is likely impossible to detect that the driving scenario is getting increasingly challenging (for instance, a snow storm approaching the vehicle) by only considering individual inputs (i.e., an image). 
%Rather, sequences of images need to be taken into account to recognize a low-confidence area of the DNN that may lead to an \textit{observable} misbehaviour (i.e., a crash). 
% may not necessarily consist of individual inputs (i.e., images), but rather of sequences of images representing an increasingly challenging driving scenario that gradually lower the confidence of the DNN leading to an \textit{observable} misbehaviour (i.e., a crash, or an out-of-bound episode (OBE) as defined in Gambi et al.~\cite{Gambi:2019:ATS:3293882.3330566}). 

%\head{Our proposal}
In this paper, we propose a novel self-assessment oracle for autonomous vehicles based on \textit{confidence estimation}, \textit{probability distribution fitting}, and \textit{time series analysis}. 
Our technique is implemented in a tool called \tool, which leverages reconstruction-based techniques from the deep learning (DL) field to analyze spatiotemporal historical driving information. The reconstruction error is used as a black-box confidence estimation for the DNN. 
During probability distribution fitting, \tool captures the behaviour of the self-driving car under nominal conditions, and fits a Gamma distribution to the observed data. Analytical knowledge of Gamma's parameters allows \tool to estimate an optimal confidence threshold, as a trade-off between prediction of all misbehaviours (the stricter the threshold, the better), and probability of false alarms (reduced when threshold is higher).
%
By observing a decreasing confidence trend over time, \tool can anticipate a misbehaviour 
%At the same time, by observing an entire time window we can get rid of noisy, spiky values, where confidence falls below threshold for a very short time.  
by recognizing unexpected conditions timely enough to enable healing actions (e.g., manual or automated disengagement). 

We have evaluated the effectiveness of \tool on the Udacity simulator of self-driving cars~\cite{udacity-simulator}, using DNNs available from the literature. 
We have modified the simulator to being able to inject unexpected driving conditions in a controllable way (i.e., day/night cycle, rain, or snow). Such injected conditions are by construction disjoint from those used to train the DNNs. 
In our experiments on 72 simulations, 
%considering both top levels of autonomy (Level~4 and~5), 
\tool is able to safely anticipate 77\% out of bound episodes/crashes, up to 6 seconds in advance. The corresponding false alarm rate in nominal driving conditions is 1\%. A comparative experiment with the online input validation strategy of DeepRoad~\cite{deeproad} shows that \tool achieves substantially superior misbehaviour prediction on all the considered effectiveness metrics (e.g., twice as high in terms of AUC-PR and almost three times higher in terms of FPR). 
%\andrea{and that DeepRoad is not applicable for online anomaly detection?} \paolo{Do we have metrics to support this claim? How long does it take for DeepRoad to measure confidence for a frame?}

Our paper makes the following contributions:

\begin{description}[noitemsep]
\item [Technique] An unsupervised technique for misbehaviour prediction based on confidence estimation, probability distribution fitting and time series analysis, implemented in the tool \tool, which is available~\cite{tool}.
\item [Simulator] An extension of the Udacity simulator to inject unexpected driving conditions dynamically during the simulation. %, as the self-driving vehicle runs.
\item [Evaluation] An empirical study  showing that the reconstruction error used by \tool for time series analysis is a promising confidence metric for misbehaviour prediction, outperforming the online input validation approach of \deeproad.
\item [Dataset] A dataset of 765 labeled simulation-based collision and out-of-bound episodes that can be used to evaluate the performance of prediction systems for autonomous driving cars.
\end{description}

%\begin{itemize}[noitemsep]
%\item An unsupervised technique for misbehaviour prediction based on confidence estimation, probability distribution fitting and time series analysis, implemented in the tool \tool, which is available~\cite{}.
%\item An extension of the Udacity simulator to inject unexpected driving conditions dynamically during the simulation. %, as the self-driving vehicle runs.
%\item An empirical study  showing that the reconstruction error used by \tool for time series analysis is a promising confidence metric for misbehaviour prediction, outperforming the input validation approach of DeepRoad.
%\item A dataset of \hl{XXX} labeled simulated-based collisions and out-of-bound episodes that can be used to  evaluate the performance of detection and prediction systems for autonomous driving cars.
%\end{itemize}


==> paper-anomaly-detection copy/2-background.tex <==
% !TEX root =  paper.tex
\section{Background}\label{sec:background}

\head{DNN-based Autonomous Vehicles}
Self-driving cars (SDC, hereafter) have benefited from many technological advancements both in hardware and in software. 
Data gathered by LIDAR sensors, cameras, and GPS are analyzed in real time by advanced Deep Neural Networks (DNN) which govern over the actual maneuvers of the car (i.e., steering, braking, acceleration).
In order to manage a wide variety of driving scenarios, SDCs necessitate a large amount of driving data, combining nominal and adversarial scenarios~\cite{10-million-miles}. %so that the SDC can learn to generalise to the conditions met everyday by human drivers.
%In fact, companies like Tesla and Google/Waymo are investing millions of dollars to collect curated datasets of driving data for training their SDCs.

To date, it is still unlikely for a DNN to generalize correctly to the plethora of driving situations met everyday by human drivers.
As such, a component monitoring the \textit{confidence} of the DNN may promptly detect when the SDC is entering a low-confidence zone, and activate healing strategies that bring the vehicle to a safe state.
% if the confidence falls below a certain acceptable value.
% Indeed, if the confidence falls below a certain acceptable value, it becomes opportune activating a mitigation strategy that can bring the vehicle to a safe state. 

In self-driving cars, depending on the level of autonomy, the self-healing procedure can either involve the human driver, or can be delegated to an automated system.\footnote{https://www.nhtsa.gov/technology-innovation/automated-vehicles-safety} 
%At NHTSA Level 4 (High Automation)\footnote{https://www.nhtsa.gov/technology-innovation/automated-vehicles-safety}, the autopilot disengages in extreme driving conditions (e.g., heavy rain/snow), and the human driver is requested to intervene. 
%At Level 5 (Full Automation -- the highest NHTSA level), all functionalities are handled automatically, including safe disengagement: e.g., an automated disengagement module may safely park the car when misbehaviours or failures are detected (e.g., a flat wheel). 
%At both top levels of autonomy, early and accurate misbehaviour prediction is an essential precondition for the overall driving system.
At both levels, early and accurate misbehaviour prediction is an essential precondition to enable safe healing, and an overall pleasant driving experience.

\head{Confidence Measures in DNNs}
The prediction must consider DNN uncertainties originating from the measurements in response to possible adverse environmental conditions in which the SDC operates. 
The confidence level of a SDC can be measured through white-box or black-box techniques. 
White-box monitoring of the internal behaviour of a DNN component. For simple classifiers, measuring softmax probabilities, or information theoretic metrics such as entropy, and mutual information~\cite{Shannon1948} may suffice. For more complex networks such as those than operate on a SDC, softmax probabilities and entropy are known to be unreliable confidence estimators~\cite{8683359}. Moreover, white-box metrics require a transparent access to the network, and substantial domain-knowledge for the creation of nontrivial probabilistic models that approximate the network's uncertainty.

Black-box techniques, differently, model the SDC uncertainty by monitoring the relation between the current input (images) and the input data used during training. For instance, consider a SDC which has been trained only with images representing highways. If images representing a narrow city street are given to the DNN, the model will still output steering angles, but ideally we would like to warn the SDC of a drop in the confidence level. The main advantages of black-box confidence metrics consist in being independent from the specific SDC architecture, requiring no modifications to the existing DNN model because they use information which is readily available for analysis, and in being, therefore, highly generalizable. %However, in our future work, we plan to investigate hybridisations of black-box and white-box techniques. 
In this paper, we focus on black-box confidence estimation, because softmax probabilities and entropy are known to be unreliable confidence estimators to model complex DNN networks~\cite{8683359}. 
%Moreover, black-box confidence metrics are independent from the specific SDC architecture, requiring no modifications to the existing DNN model, and being therefore, highly generalizable. 
%However, in our future work, we plan to investigate hybridisations of black-box and white-box techniques. 
%\paolo{We cannot just say ``We use black-box.'' without any explanation/motivation; so, I have tried to add a motivation -- feel free to strengthen it.}
%Our approach proposes a reconstruction-based approach that employs a predictively trained model of normality. 
%The problem of detecting unexpected driving conditions to predict possible misbehaviours throughout the driving time is related to unsupervised deep learning-based anomaly detection and time series analysis. Both research areas have a broad literature; for conciseness, we limit our background to those approaches that are relevant for our proposal. Particularly, 
We next describe autoencoders and time series analysis, which are the main building blocks of our approach. 

\begin{figure*}[t]
\centering
%\fbox{
%\includegraphics[trim=0cm 10cm 1cm 0cm, clip=true,scale=0.15]{images/example-2}
\includegraphics[trim=0cm 10cm 1cm 0cm, clip=true,width=0.8\textwidth]{images/example-2.pdf}
%}
\caption{Confidence levels of NVIDIA's DAVE-2~\cite{nvidia-dave2} in response to changing driving scenarios. 
The picture shows frames captured during the execution of the SDC along one of our testing tracks, under different conditions: (Lap~1)~sun, (Lap~2)~light rain, (Lap~3)~sun, and (Lap~4)~heavy rain.
The picture juxtaposes the reconstruction error by the anomaly detector of \tool, which is used as a proxy for the DNN confidence.
We can notice that the reconstruction error is low when the car drives under sunny conditions (i.e., conditions similar to those observed during training), whereas the error increases moderately with adverse conditions (the car does no longer follow the center of the road), and grows above a given threshold when facing heavy rainy conditions at night time (which cause the SDC to drive off the road).} 
\label{fig:example} 
\end{figure*}

\head{Autoencoders}\label{sec:autoencoders}
An autoencoder (AE) is a DNN designed to reconstruct its own input. It consists of two sequentially connected components (an encoder, and a decoder) that are arranged symmetrically. % (\autoref{fig:ae}).
The simplest form of autoencoder (SAE) is a three-layer DNN: the input layer, the hidden layer, and the output layer.
The hidden layer encodes any given input $\boldsymbol{x} \in \mathcal{R}^{D}$  to its internal representation (\textit{code}) $\boldsymbol{z} \in \mathcal{R}^{Z}$ with a function
$f(\boldsymbol{x}) = \boldsymbol{z}$. Usually $Z \ll D$.
The output layer (decoder) decodes the encoded input with a reconstruction function $g(\boldsymbol{z}) = \boldsymbol{x'}$, where $\boldsymbol{x'}$ is the reconstructed input $\boldsymbol{x}$. 
The autoencoder minimises a loss function $\mathcal{L}(\boldsymbol{x}, g(f(\boldsymbol{x})))$, which measures the distance between the original data and its low-dimensional reconstruction. A widely used loss function in autoencoders is the Mean Squared Error (MSE).

%$$
%\mathcal{L}(\boldsymbol{x}, \boldsymbol{x'}) = \displaystyle\frac{1}{n}\sum_{t=1}^{n}\lVert \boldsymbol{x} - \boldsymbol{x'} \rVert^2
%$$

%\begin{figure}[t]
%\centering
%%\fbox{
%\includegraphics[trim=0cm 7cm 1cm 0cm, clip=true,scale=0.14]{images/autoencoder.pdf}
%%}
%\caption{Architecture of autoencoders.} 
%\label{fig:ae} 
%\end{figure}

%\subsubsection{Autoencoder Architectures}
The input and output layers of autoencoders have the same number of nodes. If multiple hidden layers are used, the architecture is referred to as deep autoencoder (DAE). %The size $\boldsymbol{Z}$ of the innermost (\textit{latent}) representation can also vary.
The surge of novel kinds of DNNs has correspondingly produced variants of autoencoders based on such architectures. For example, 
%deep autoencoders~\cite{Vincent:2010:SDA:1756006.1953039} (), 
convolutional autoencoders~\cite{10.1007/978-3-642-21735-7_7}
allow learning powerful spatial-preserving relationship within images at a lower training time with respect to fully dense layers.
Another interesting proposal are variational autoencoders (VAE) that are able to model the relationship between the latent variable $\boldsymbol{z}$ and the input variable $\boldsymbol{x}$ by learning the underlying probability distribution of observations using variational inference~\cite{An2015VariationalAB}.


% extract relevant features from the input image using convolutional layers. Combined with nonlinear activation functions, convolutional layers allow learning powerful representations while substantially lowering the training time with respect to fully dense layers.
%denoising autoencoders~\cite{VincentLLBM10}, 
%and variational autoencoders~\cite{An2015VariationalAB}.
%
%Deep autoencoders (DAE)~\cite{Vincent:2010:SDA:1756006.1953039} follow the general architecture shown in \autoref{fig:ae} and described above.
%The main distinguishing trait of Convolutional autoencoders (CAE)~\cite{10.1007/978-3-642-21735-7_7} is that they extract relevant features from the input image. 
%During training, convolutional layers learn spatial-preserving relationship between pixels by sliding a small window across the input image. %Extracted features are only dependent on a small neighbouring region with the size of this window. Combined with nonlinear activation functions, convolutional layers allow learning powerful representations while substantially lowering the training time with respect to fully dense layers.
%
%Variational autoencoders (VAE)~\cite{An2015VariationalAB} are able to model the relationship between the latent variable $\boldsymbol{z}$ and the input variable $\boldsymbol{x}$ by learning the underlying probability distribution of observations using variational inference. 
%The loss function of VAE consists of two terms: (1) the expected value of the negative log-probability of the input $\boldsymbol{x}$ given the code $\boldsymbol{z}$; (2) the Kullback-Leibler divergence between the distribution of $\boldsymbol{z}$ given  $\boldsymbol{x}$ and the distribution of $\boldsymbol{z}$ alone. The first term plays the role of the reconstruction loss reduction, since it maximises the probability of getting the input from the code. The second term forces the VAE to minimise information loss in the latent space, hence avoiding that similar inputs are mapped to distant regions of the latent space.

%\subsubsection{Autoencoder for Anomaly Detection}
%
%We are interested in AEs for the special properties of the latent variable $\boldsymbol{z}$. The networks can be trained to prioritize learning the fraction of the input that is worth considering for the task at hand. 
%
%In our case of recognizing suspicious frame images, autoencoders are trained only on data with normal instances, thus learning learn how to accurately reproduce the most frequent characteristics. When facing previously unseen samples (anomalies), the model should worsen its reconstruction performance~\cite{An2015VariationalAB}. 
%Reconstruction error of a data point is the error between the original data point and its low dimensional reconstruction, defined as
%$\boldsymbol{e}^{i} = (\boldsymbol{x} - \boldsymbol{x'})^2$.
%
%Typically, it is either adopted as an anomaly score to detect anomalies, or used to estimate the parameters $\mu$ and $\Sigma$ of a Gaussian distribution $\mathcal{N}(\mu, \Sigma)$ using maximum likelihood estimation (MLE). For example, the anomaly score for a point $x^{i}$ could be defined as:
%
%$$
%a^{i} = (\boldsymbol{e}^{i} - \mu)^T  \Sigma^{-1}(\boldsymbol{e}^{i} - \mu) $$ 
%
%%$$
%%\boldsymbol{e}^{i} = (\boldsymbol{x} - \boldsymbol{x'})^2
%%$$

%\begin{figure}[t]
%\centering
%%\fbox{
%\includegraphics[trim=0cm 0cm 0cm 0cm, clip=true,scale=0.20]{images/RNN-unrolled.png}
%%}
%\caption{Time unrolling of a recurrent neural network. 
%\paolo{We do not have copyright on this image, so we have to replace it with our own image.}} 
%\label{fig:lstm} 
%\end{figure}




\head{Time Series Analysis}\label{sec:rnn}
Traditional feedforward DNNs assume that all inputs and outputs are independent of each other. However, learning temporal dependencies between inputs or outputs is important in tasks involving continuous streams of data. 
Thus, a predictive model can take advantage of information from the previous inputs/outputs, to enhance its predictive capability.

Time series analysis can be applied to the output sequence produced by a DNN to identify the trend and predict future values. Among the numerous models available for time series analysis, the most widely used ones are autoregressive (AR), integrated (I) and moving average (MA) models, along with their combinations. An AR model of order $k$ predicts the next value $x_t$ as a linear combination of past values $x_{t-1}, \ldots, x_{t-k}$:

\begin{equation} \label{eq:ar}
x_t = \alpha_0 + \sum_{i = 1}^k{\alpha_i x_{t-i}} + \epsilon_t
\end{equation}

\noindent
where coefficients $\alpha_0, \ldots, \alpha_k$ can be estimated by the least square method and $\epsilon_t$ represents the error term.

%\head{Long-Short Term Memory (LSTM)}
Processing of a sequence of inputs can be achieved by recurrent neural networks (RNN) equipped with long short-term memory (LSTM)~\cite{Hochreiter:1997:LSM:1246443.1246450}, which is capable of dealing with both short and long range dependencies. 
In LSTM, outputs are influenced not only by the current input but also by the state of the RNN, which encodes the entire history of past inputs. A \textit{forget gate} layer of LSTM decides what information to keep/remove from the previous network state whereas an \textit{additive gate} decides how to update the state based on the current input. 
%\autoref{fig:ae} shows the general state feedback mechanism of RNN and its unrolling over time, hiding the details of the LSTM gates inside block $A$.

%% OLD ANOMALY DETECTION
%\subsection{Anomaly Detection}
%
%Anomaly detection is a challenging and multi-faceted problem that has been studied thoroughly within a multitude of research areas and application domains such as intrusion detection systems~\cite{7987197,7906980,8416441}, fraud~\cite{FIORE2019448,8311689,GOMEZ2018175} and malware detection~\cite{Yuan:2014:DDL:2619239.2631434,7280815,7814490},  social networks~\cite{DBLP:journals/corr/abs-1902-06673,Ruchansky:2017:CHD:3132847.3132877}, and internet of things~\cite{7474197}. 
%At a high level, an \textit{anomaly} (or \textit{outlier}) can be defined as an observation that significantly deviates from other observations so as to arouse suspicion that it was generated by a different mechanism~\cite{DBLP:journals/corr/abs-1901-03407,GVK02435757X}.
%Anomalies can be caused by errors in the data but they can be also indicative of new, previously unknown, underlying scenarios. 
%
%When labeled abnormal instances are available (i.e., in a \textit{supervised} context), classical machine learning approaches such as support vector machines (SVM)~\cite{6943078}, $k$-nearest neighbour~\cite{Ando:2015:EAD:2725270.2725380}, or random decision forests~\cite{Ho95} have shown good results.
% 
%However, in many real world domains, such as autonomous driving, abnormal data represent rare and unexpected events, for which  no prior knowledge, or label, is available (hence, the context is \textit{unsupervised}). 
%Thus, research has moved to models that can be trained using no supervision, including one class SVM~\cite{ScholkopfWSSP99}, clustering~\cite{Everitt2009} and self-organizing maps~\cite{Kohonen01}.

% OLD FIGURE
%\begin{figure*}[t]
%\centering
%%\fbox{
%\includegraphics[trim=0cm 16cm 0cm 0cm, clip=true,scale=0.199]{images/example}
%%}
%\caption{Confidence levels of NVIDIA's DAVE-2~\cite{nvidia-dave2} in response to changing driving scenarios. The picture shows the stream of frames captured during the execution of the SDC along one of our testing tracks, under three different conditions: (top)~``normal'' sun, (middle)~light rain, (3)~heavy rain. Numbers below each frame denote the reconstruction error by the anomaly detector of \tool, which is used as a proxy for the DNN confidence. 
%We can notice that the reconstruction error is low when the car drives under ``normal'' sunny conditions (i.e., conditions similar to those observed during training), whereas the error increases with moderately adverse conditions (the car does no longer follow the center of the road), and heavy rainy conditions at night time cause the DNN to drive off the road. \andrea{find better images}} 
%\label{fig:example} 
%\end{figure*}



==> paper-anomaly-detection copy/3-problem.tex <==
\section{Problem formulation}\label{sec:problem}

%Simulators for autonomous driving systems, such as BeamNG~\cite{beamng} or CARLA~\cite{carla}, allow testing of SDCs by providing out-of-the-box rule- and reinforcement learning-based autonomous driving agents. 
%Differently, in this paper we consider DNN-based SDCs that learn from multiple driving examples through training, and are then deployed on actual vehicles. 
%For instance, models by NVIDIA~\cite{nvidia-dave2} or the Udacity self-driving challenge~\cite{udacity-challenge} are DNNs that solve a supervised regression problem between the car steering angles and the road images in front of the car.

We focus on SDCs that perform \textit{behavioural cloning}, i.e., the DNN learns the \textit{lane keeping}~\cite{Gambi:2019:ATS:3293882.3330566} behaviour from a human driver.
Models such as the ones by NVIDIA~\cite{nvidia-dave2} or the Udacity self-driving challenge~\cite{udacity-challenge} are trained with visual inputs (i.e., images) from car-mounted cameras that record the driving scene, paired with the steering angles from the human driver. The DNN then ``learns how to drive'' by discovering underlying patterns within the training images representing the shape of the road, and predicting the corresponding steering angle. 
% (brake/acceleration values could also be learned from the data, but it is quite common to define an analytical method to compute them from the steering angle that does not require training). 
%Since it is practically impossible to make sure that all possible driving conditions are represented in the training set, automated online recognition of unexpected conditions is an important component of DNN-based self-driving cars to ensure a safe behaviour even in such situations.

%\subsection{Characterization of Misbehaviours in Autonomous Driving Systems}\label{sec:definition-misbehaviours}

\begin{figure*}[t]
\centering
%\fbox{
\includegraphics[trim=0cm 23cm 0cm 0cm, clip=true,scale=0.20]{images/training.pdf}
%}
\caption{Model Training under Nominal Driving Behaviour.} 
%\paolo{The name of the threshold is $\theta$, not $\eta$.}
\label{fig:approach} 
\end{figure*}

%A misbehaviour is a failure of the DL system in response to underrepresented/unexpected inputs. 
For a classification problem (e.g., hand-written digit recognition), a misbehaviour can be defined as an input that can be confidently labeled by humans while it is misclassified by a DNN. 
%Differently, for a regression problem (e.g., steering angle prediction) such a definition is more troublesome, because there is no expected outcome for an individual output of the DNN and it is only the overall behaviour resulting from the DNN predictions that may or may not be acceptable, depending on the specific application domain. In autonomous driving, it is not possible to decide if an individual prediction of the steering angle is a mis-behaviour, while a sequence of steering angle predictions that lead to a crash is is more likely to lead to a mis-behaviour. In other words, the notion of mis-behaviour descends from the overall expected behaviour of the system, i.e., from the \textit{requirements} that the system containing the DNN is supposed to implement.
Differently, for a regression problem %(e.g., steering angle prediction) 
such a definition is more troublesome, because there is no expected outcome for an individual output of the DNN and it is only the overall behaviour resulting from the DNN predictions that may or may not be acceptable, depending on the specific application domain.

In steering angle prediction, it is challenging to decide if the steering angle produced by a DNN is wrong, because the optimal steering angle is generally unknown for a new test scenario and even if it were known, the amount of difference between predicted and expected steering angle that qualifies as an error is difficult to decide a priori. It is instead more realistic to figure out whether a chain of inaccurate predictions, regardless of the amount of deviation from the optimal angles, ultimately leads to a misbehaviour of the system. 
%First, the complex decision making process of DNNs makes extremely difficult to understand and characterize their exact behaviour.
%Second, the learning component of DNNs is what makes them special w.r.t. learning from data in order to solve hard problems (other than let developers coding the behaviour within the system such as classical rule-based AI systems). 


In fact, the  definition of misbehaviour should be decoupled from the notion of correct/wrong DNN output, being instead linked to the ability of a DNN of abstracting from the training examples and learning how to drive in different ways/conditions. 
%In fact, in principle, there is no single ``correct'' steering angle for a single bend, despite the training set should be sufficiently representative of a number of different situations. 
It is the task of the DNN to  generalize the training knowledge to make the model robust w.r.t. slightly different conditions from those observed in the training set.
For instance, if the SDC is facing a 90-degree bend, the DNN may decide to steer at a certain steering angle $\theta$ if the car speed is 60 mph, or $\frac{\theta}{2}$ if the speed is 30 mph.
%Indeed, the tradeoff between DNNs training cost, generalization and understandability remains an open issue.

\begin{defn}[\textbf{Misbehaviour of a DNN}]
A DNN exhibits a \textit{misbehaviour} in a given test scenario if the overall system that contains the DNN does not respect its requirements due to the outputs produced by the DNN.
\end{defn}

In the autonomous driving domain, there are many possible misbehaviours, associated with the different requirements that such systems are supposed to realize. Safety requirement violations are by far the most critical requirements, as a misbehaviour in the steering component may cause a crash of the vehicle with potential casualties.
However, in general, a SDC might violate also other driving requirements, e.g., related to ride comfort~\cite{10.1007/978-3-658-21194-3_53}, such as excessive derivative of the steering angle, unstable movement around the centerline, or excessive deceleration. All these could also be considered as misbehaviours by our definition.





In this paper, we focus on the prediction of two safety-critical misbehaviours: (1)~collisions, and (2)~out-of-bound episodes (OBEs). 
The rationale for this choice are as follows. 
First, they represent the vital requirement to be satisfied and thoroughly tested (i.e., the car should stay in lane and avoid whatsoever collision), without which autonomous driving vehicles would be hardly accepted in production.
Moreover, leveraging a simulation environment such as Udacity's~\cite{udacity-simulator}, allows us to: (1)~safely test such critical scenarios, (2)~precisely define, observe and measure them, in order to support crash analysis and reproduction.

Thus, the \textbf{\textit{problems}} we want to address in this paper are: (1)~recognizing when a self-driving car is within a low-confidence area because of an unexpected execution context, and (2)~predicting such situation timely enough so as to take countermeasures before the vehicle may crash or drive off road.

%PAOLO: this section should end with problem formulation; what we do and why it's novel is not in the scope of this section
%We conjecture that prediction of such misbehaviours can be tackled by time series analysis of the data ``seen'' by the ego car and by early detection of unexpected frames that signal a low-confidence area for the DNN (see \autoref{fig:example}). To the best of our knowledge, this is the first paper that aims at \textit{predicting} misbehaviours, rather that detecting them after they have already occurred, e.g., by classifying them as anomalous~\cite{deeptest,deeproad,deepxplore}.



==> paper-anomaly-detection copy/4-approach.tex <==
%% !TEX root =  paper.tex

%\begin{figure*}[t]
%\centering
%%\fbox{
%\includegraphics[trim=0cm 16cm 18cm 0cm, clip=true,scale=0.25]{images/approach-new.pdf}
%%}
%\caption{Mis-behaviour prediction in DNN-based autonomous driving systems.} 
%\label{fig:approach} 
%\end{figure*}

\section{Approach}\label{sec:approach}

%Predicting unexpected scenarios during the motion of the vehicle makes analyzing the datasets in autonomous driving research more challenging than techniques that identify single underrepresented images in the training set. 
%To face this challenge, our approach combines a DL reconstruction-based anomaly detector to construct a predictively model of normality based on time series analysis.

The goal of our approach is to monitor the confidence level of a SDC as it runs and to promptly predict whether drops in confidence correlate with potential future misbehaviours. 
%Our focus is on the mis-behaviours classes described in \autoref{sec:definition-misbehaviours}, i.e, collisions and OBEs.
Our approach works in an end-to-end fashion, analyzing directly the input data as retrieved by the car (an image from the center camera), making the approach independent from the specific architecture of the self-driving component, requiring no modifications to the existing DNN model, and being therefore, highly generalizable.

The main working assumption is that a prediction model trained on normal data should learn the normal time series patterns. When the model is used on a SDC in the field, it should worsen its performance as the car approaches previously unseen regions as compared to normal, known regions (\autoref{fig:example}). Then, what's needed is a way to set up a good decision boundary in order to timely alert the human driver (NHTSA Level~4) or the main self-driving component (NHTSA Level~5) about triggering self-healing. 

We now detail each step of our approach, which consists of two main phases: (1)~\textit{model training under nominal driving behaviour}, and (2)~\textit{field usage of the trained model}.

\subsection{Training of \tool under Nominal Driving Behaviour}\label{sec:training}

\autoref{fig:approach} illustrates the training phase of our approach, which consists of several steps. 

\subsubsection{Reconstructor}

The first step consists in retrieving a model of normality from the training driving scenarios. Thus, in the training set, we capture the visual input stream of the SDC under nominal situations.

%PAOLO: the following is a contingent experimental choice (normal = sunny; anomalous = not sunny), but another experiment could be with normal = sunny + rainy + dark an anomalous = something else, so I would not define normality based on the experimental choices
%In our simulation-based setting, normality consists of driving records representing (1)~smooth driving conditions over (2)~a known track, (3)~with sunny weather conditions. However, if available, any training set that was used to train a generic SDC can be adopted.

Then, we train our driving scenario reconstructor with such ``normal'' instances.
Let us consider a training set $\boldsymbol{X} = \{x_1, x_2, \ldots, x_n \}$ of $n$ image frames, where the index $i \in [1:n]$ of $x_i \in \boldsymbol{X}$ represents the discrete time $t$. 
%The reconstructor reads each image $x_i \in \boldsymbol{X}$, and attempts to reconstruct $x'_i$ with high fidelity.

Depending on the considered architecture, a reconstructor can be \textit{singled-image} or \textit{sequence-based}. 
For singled-image reconstructors, only one image frame is considered at a time. When the discrete time is $t = i$, $x_i$ is the input and the reconstructor recreates it into $x'_i$. 
For sequence-based reconstructors, assuming $k$ image frames preceding $x_i$ are used to reconstruct $x_i$, the sequence 
$\langle x_{i-k}, \ldots, x_{i-1}\rangle$ is the input used to output $x'_i$, a prediction of the actual current frame $x_i$.
For instance, for $k=3$ and $i = 4$, the reconstructor considers the sequence $\langle x_1, x_2, x_3 \rangle$ in order to predict the current frame $x_4$.

At the end of this task, each reconstruction error $e_i=d(x_i, x'_i)$ can be computed, where $d$ is a proper distance function (e.g., Euclidean distance). This results in the set of reconstruction errors $\boldsymbol{E} = \{e_1, e_2, \ldots, e_n \}$, available for all elements in the training set $\boldsymbol{X} = \{x_1, x_2, \ldots, x_n \}$.



\begin{figure}[b]
\centering
\fbox{
\includegraphics[trim=0cm 15cm 11cm 0cm, clip=true,scale=0.35]{images/histogram-gamma.pdf}
}
\caption{Fitted Gamma distribution of reconstruction errors from a VAE on the Dave2 dataset.} 
\label{fig:hist} 
\end{figure}

\subsubsection{Probability Distribution Fitting}

We build a model of normality for the reconstruction errors $\boldsymbol{E} = \{e_1, e_2, \ldots, e_n \}$ collected in nominal driving conditions.
We use probability distribution fitting to obtain a statistical model of normality and using such model we determine a threshold $\theta$ that brings the expected false alarm rate in nominal conditions below some acceptable, configurable level $\epsilon$ (e.g., $\epsilon = 10^{-3}$ or $\epsilon = 10^{-4}$).

%PAOLO: at the pixel level, we also assume that the error distribution is Gaussian
%Unlike existing works on time series analysis, we do not assume a known underlying distribution of the reconstruction errors, such as a Gaussian distribution.
%Indeed, earlier work have shown that thresholding assuming Gaussian distribution may result in suboptimal precision and recall results.
%Thus, first we used D'Agostino and Pearson's normality test~\cite{dagostino} to reject the null hypothesis of normality for all reconstruction error sets using a threshold $\alpha = 0.05$. 

The reconstruction error $e = d(x, x')$ can be computed by comparing the individual pixels of the images $x$ and $x'$ and taking the mean pixel-wise squared error. Assuming images have width $W$, height $H$ and $C$ channels (usually, 3 RGB channels for colour images), the reconstruction error is defined as follows:




\begin{equation}
d(x, x') = \frac{1}{W H C} \sum_{i = 1, j = 1, c = 1}^{W, H, C}{(x[c][i, j] - x'[c][i,j])^2}
\end{equation}

With some reasonable approximation, we can assume that the pixel-wise error $e[c][i, j] = x[c][i, j] - x'[c][i,j]$ follows a normal distribution with pixel dependent variance: $e[c][i, j] \sim \mathcal{N}(0, \sigma_{c, i, j})$. Correspondingly, the sum of the squares of pixel-wise errors $e[c][i, j]$ will be a gamma distribution: $e = d(x, x') \sim \Gamma(\alpha, \beta)$. We get a gamma instead of a $\chi^2$ distribution because pixel-wise errors have different (channel/pixel dependent) and non-unitary variances.

%The mean of squared reconstruction errors  follows a Gamma distribution. 
%Indeed, the reconstruction error set $\boldsymbol{X}$ is distributed normally with mean $\mu = 0$ and variance $\sigma = 1$ ($e_i \in \mathcal{N}(0, 1)$). Then, it follows that the squared of $\boldsymbol{X}$ fits a chi-squared distribution 
%
%$$ \sum_{i} e_i^2 \sim \tilde{\chi}^2 $$
%
%However, if $\boldsymbol{X}$ is not normally distributed ($e_i \in \mathcal{N}(0, \sigma)$), such as the MSE, then $\boldsymbol{X}$ follows a Gamma distribution 
%
%$$
%\sum_{i} e_i^2 \sim \Gamma
%$$

\head{Definition of  Gamma Distribution}
Gamma is a probability model for a continuous variable on $[0,\infty)$ which is widely used in engineering, science, and business, to model continuous variables that are always positive and have skewed distributions. 

The \textit{probability density function} of a random variable $x\sim\Gamma(\alpha, \beta)$ is:

\begin{equation}\label{eq:pdf-gamma}
f(x)=\frac{\beta^{\alpha}}{\Gamma(\alpha)}x^{\alpha-1}e^{-\beta x} 
\hspace{.2in} x > 0; \ \alpha, \beta > 0
\end{equation}

\noindent
where $\alpha$ is the \textit{shape} parameter (which affects the shape of the distribution), $\beta$ is the \textit{rate} parameter (or inverse scale, which stretches/shrinks the distribution) and $\Gamma$ is the gamma function. 
When $\alpha$ is large, the gamma distribution closely approximates a normal distribution with the advantage that the gamma distribution has non-zero density only for positive real numbers.



The \textit{gamma function} $\Gamma$ can be seen as a solution to the interpolation problem of finding a smooth curve that connects the points  $(n, m)$ with $m = (n-1)!$ at any positive integer value for $n$. 
Such a definition was extended to all complex numbers with a positive real part by Bernoulli, as a solution to the following integral:

\begin{equation}\label{eq:gamma}
\Gamma(z) = \int_{0}^{\infty} {x^{z-1}e^{-x}dx} 
\hspace{.2in}  \mathfrak{R}(z) > 0;
\end{equation}


\begin{figure*}[t]
\centering
%\fbox{
\includegraphics[trim=0cm 27.5cm 3cm 0cm, clip=true,scale=0.205]{images/testing.pdf}
%}
\caption{Usage Scenario of \tool. 
} 
\label{fig:testing} 
\end{figure*}





%\head{Fitting the Gamma Distribution}
%Fitting distributions to data consists of choosing a probability distribution for the data, as well as finding parameter estimates for that distribution~\cite{JSSv064i04}. 
%The choice may be guided by the knowledge of stochastic processes governing the modelled variable, or, alternatively, by the observation of its empirical distribution (see \autoref{fig:hist}). 






%In addition to empirical plots, descriptive statistics can help discriminate the best candidates based on quantitive measures of fitness. For instance, a used approach concerns evaluating the skewness and kurtosis values. 
%A non-zero skewness reveals a lack of symmetry of the distribution, whereas the kurtosis value quantifies the weight of tails in comparison to the normal distribution for which the kurtosis equals 3. Nonparametric bootstrap procedure is used to mitigate the uncertainty of the estimated values.
%For example, for the VAE, the value of skewness is $1.586735$, whereas the value of kurtosis is $6.687906$.
%\autoref{fig:graph} shows the results on our VAE example with a positive skewness and a kurtosis not far from 3 after a nonparametric bootstrap procedure used to mitigate the uncertainty of the estimated values (boot=500).
%We can notice how the fit of three common right-skewed distributions (Weibull, Gamma and Lognormal distributions) could be considered to fit the error distribution.

%\begin{figure}[h]
%\centering
%%\fbox{
%\includegraphics[trim=0cm 15cm 12cm 0cm, clip=true,scale=0.4]{images/graph.pdf}
%%}
%\caption{Skewness-kurtosis plot of a distribution of reconstruction errors from the VAE on Dave2 dataset.} 
%\label{fig:graph} 
%\end{figure}

%However, skewness-kurtosis plots should then be regarded as indicative only. Skewness and kurtosis are not considered robust because of their high variance, which cannot be completely solved by the use of bootstrap. 
%Thus, we considered an alternative method consisting in maximizing likelihood estimation, which we describe next.

%summary statistics VAE loss
%------
%min:  43.56643   max:  62.6084 
%median:  52.54897 
%mean:  52.60987 
%estimated sd:  6.328202 
%estimated skewness:  1.586735 
%estimated kurtosis:  6.687906 

% VAE Loss
%Fitting of the distribution ' gamma ' by maximum likelihood 
%Parameters : 
%       estimate Std. Error
%shape 69.498103 4.38470666
%rate   1.321022 0.08364526
%Loglikelihood:  -1628.238   AIC:  3260.477   BIC:  3268.906 
%Correlation matrix:
%          shape      rate
%shape 1.0000000 0.9964046
%rate  0.9964046 1.0000000

\head{Fitting the Gamma Distribution}
One powerful method to estimate the parameters of a (gamma) distribution that fit the data (reconstruction errors) best is by maximum likelihood estimation (MLE). The likelihood function reverses the roles of the variables: in \autoref{eq:pdf-gamma}, the values of $x$ are known, so they are the fixed constants, whereas the unknown variables are the parameters $\alpha$ and $\beta$. MLE involves calculating the values of these parameters so as to obtain the highest likelihood of observing the values of $x$ when the given parameters are supplied to $f$.

Under the assumption of independence of the data, the likelihood of the data given the parameters of the distribution is conveniently defined as the logarithm of the joint probability of the data for a given choice of the parameters. In the case of a gamma distribution, with a dataset consisting of reconstruction errors $\boldsymbol{E} = \{e_1, e_2, \ldots, e_n \}$, we get:

\begin{eqnarray} \label{eq:maxlike}
\mathcal{L}(\alpha, \beta; \boldsymbol{E}) = \frac{1}{n}\sum_{i=1}^n{\log f(e_i | \alpha, \beta)} = \\
  n (\alpha-1)\overline{\log e} - n \log \Gamma(\alpha) - n \alpha \log \beta - n \overline{e} / \beta
\end{eqnarray}

\noindent
where $\overline{e}$ ($\overline{\log e}$) is the mean (log) reconstruction error over $\boldsymbol{E}$.
To find the values of parameters $\alpha$ and $\beta$ that maximize $\mathcal{L}$ we have to find a solution to the equations: 
(1) $\partial \mathcal{L} / \partial \alpha = 0$; (2) $\partial \mathcal{L} / \partial \beta = 0$.
%
%\begin{equation} \label{eq:mle-deriv}
%\frac{\partial \mathcal{L}}{\partial \alpha} = 0;
%\frac{\partial \mathcal{L}}{\partial \beta} = 0
%\end{equation}
%
The second equation can be easily solved analytically, resulting in $\beta = \overline{e} / \alpha$. By substituting the value of $\beta$ into the first equation we get an equation that unfortunately cannot be solved analytically. However, the Newton method can iteratively converge to the solution quite quickly. The output of such numerical estimation will be the pair of parameters $\alpha$ and $\beta$ of the gamma distribution that best fit the reconstruction errors.

%The likelihood has the same form as the gamma probability density function (\autoref{eq:pdf-gamma}) for which the parameters $\alpha$ and $\beta$ are known constants and the variable to determine is $x$. 


%\head{Fit of Gamma Distribution by Maximum Likelihood Estimation}
%Essentially, the key to calculating maximum likelihood estimators is to remove factors that are constant with respect to the parameter to be maximized.
%For the parameters of the Gamma, shape and rate (i.e., $\alpha$ and $\beta$ in \autoref{eq:pdf-gamma}), are computed maximizing a likelihood function~\cite{mle-gamma} as follows.

%\begin{equation}\label{eq:likelihood-gamma}
%\mathfrak{L}(\theta) = \prod_{i=1}^{n} f(x_i | \theta) 
%\end{equation}

%In the case of Gamma, the maximum likelihood estimation method is used to estimate shape and rate (i.e., $\alpha$ and $\beta$ in \autoref{eq:pdf-gamma}) according to the following procedure. 

% https://math.stackexchange.com/questions/1510480/mle-of-%CE%B2-in-the-gamma-distribution
%For a sample $\boldsymbol{x} = (x_1, \dots, x_n)$ with observations $x_i \sim \Gamma(\alpha,\beta)$, where the shape $\alpha$ and the rate $\beta$ are unknown, we have the joint distribution
%
%$$
%f(\boldsymbol x \mid \alpha,\beta) = \prod_{i=1}^n f(x_i \mid \alpha,\beta) = \left( \frac{\beta^\alpha}{\Gamma(\alpha)} \right)^n \prod_{i=1}^n x_i^{\alpha-1} \exp(-\beta x_i) \propto \beta^{n \alpha} \exp\left(-\beta \sum_{i=1}^n x_i \right).
%$$
%
%For instance, if we are interested in the likelihood of $\beta$ with respect to fixed $x$ and $\alpha$, we remove all factors that are not functions of $\beta$.
%Thus the log-likelihood of $\beta$ is proportional to
%
%$$
%\ell(\beta \mid \alpha, \boldsymbol x) \propto n \alpha \log \beta - \beta n \bar x \propto \alpha \log \beta - \bar x \beta.
%$$
%
%The log-likelihood has critical points for $\beta$ satisfying
%
%$$
%0 = \frac{\partial \ell}{\partial \beta} = \frac{\alpha}{\beta} - \bar x,
%$$
%
%therefore 
%
%$$
%\hat \beta = \frac{\alpha}{\bar x}
%$$
%
%is a critical point. Since in $\ell(\beta \mid \alpha, \boldsymbol x)$ the derivative is strictly negative for $\beta > 0$ , it follows that the critical point $\hat \beta$ is a global maximum of the likelihood function and is therefore the MLE.
%Similar reasoning applies to estimating the MLE for $\alpha$.
%
% https://www.math.arizona.edu/~jwatkins/O3_mle.pdf
%First, given the parameter $\alpha$ and $\beta$, we define the \textit{likelihood function} of the Gamma probability density function (\autoref{eq:pdf-gamma}) as:
%
%\begin{equation}\label{eq:likelihood-gamma}
%\mathfrak{L}(\alpha, \beta | \boldsymbol{x}) = \sum_{n=0}^{N-1} log P(x_{n}) 
%\end{equation}
%
%and its logarithm
%
%\begin{equation}\label{eq:log-likelihood-gamma}
%ln \mathfrak{L}(\alpha, \beta | \boldsymbol{x}) = n(\alpha ln \beta - ln \Gamma(\alpha)) + (\alpha + 1) \sum_{i=1}^{n} ln x_i - \beta \sum_{i=1}^{n} x_i
%\end{equation}
%
%The score function is a vector 
%( $\frac{\partial}{\partial \alpha} ln \mathfrak{L}(\alpha, \beta | \boldsymbol{x}$), 
%$\frac{\partial}{\partial \beta} ln \mathfrak{L}(\alpha, \beta | \boldsymbol{x}))$
%in which the zero components determine the maximum likelihood estimators. Thus, to determine these parameters, we solve the equations

\head{Example of Threshold Estimation}
Let us consider a set of reconstruction errors. \autoref{fig:hist} shows the histogram of those produced on the Dave2 dataset when the reconstructor is a VAE. On such dataset the MLE method estimates the following gamma parameters: $\alpha = 15$; $\beta = 392$. With these parameter values, the plot of the gamma distribution is the red line in \autoref{fig:hist}. We can notice a good agreement between the histogram and the estimated probability distribution.

Let us assume that we are willing to accept a false alarm rate $\epsilon = 10^{-2}$. The threshold $\theta$ with a probability mass above the threshold equal to $10^{-2}$ can be easily obtained as the inverse of the cumulative gamma distribution $F(x)$: $\theta = F^{-1}(1-\epsilon)$. This ensures that the cumulative probability of values $\leq \theta$ is $1-\epsilon$, leaving only a probability of $\epsilon$ to the tail following $\theta$. 
%With reference to \autoref{fig:hist}, when $\epsilon = 10^{-3}$ (resp. $10^{-4}$ or $10^{-5}$) we get $\theta$ = \hl{VV} (resp. \hl{VV} or \hl{VV}). 
We use the estimated $\theta$ as threshold to distinguish anomalous conditions (reconstruction error $\geq \theta$) from normal ones (reconstruction error $< \theta$). 

%print("Fitting Gamma using scipy.stats")
%shape, loc, scale = gamma.fit(losses, floc=0)
%print("shape, loc, scale", shape, loc, scale)
%y = gamma.pdf(losses, shape, loc, scale)
%print(y)
%print(gamma.ppf([0.68, 0.90, 0.95, 0.99, 0.999, 0.9999], shape, loc=loc, scale=scale))
%Let us consider a distribution of random numbers from the gamma distribution with 
%$\alpha = 10$ and $\beta = 5$. The confidence intervals can be calculated using the percent point function ppf. The MLE for parameter $\alpha$ is 10.98, compared to the true value of 10. Thus, the 95\% confidence interval for $\alpha$ goes from 7.4 to 14.6, which includes the true value.
%
%Similarly the MLE for parameter $\beta$ is 4.7, compared to the true value of 5. The 95\% confidence interval for $\beta$ goes from 3.2 to 6.3, which also includes the true value.
%In our setting, we do not know the true value of $\alpha$ and $\beta$, so the MLE method allows us to have a confidence interval on the parameters to give a range of likely values.

%\subsection{Time-series-based Misbehaviour Prediction}


%In this paper, we only consider image frames from a center-mounted camera. 
%A driving scenario can be then abstractedly represented as a data stream $\mathcal{DS}$, defined as $\mathcal{DS} = \{ \boldsymbol{x}^{(1)}, \boldsymbol{x}^{(2)}, \boldsymbol{x}^{(3)}, \boldsymbol{x}^{(3)}, \ldots, \boldsymbol{x}^{(n)}, \ldots \} $ 
%where each point $\boldsymbol{x}^{(t)} \in R^{m}$ in the time series is an $m$-dimensional vector $\{ {x}_1^{(t)}, {x}_2^{(t)}, \ldots,  {x}_m^{(t)} \}$ representing the image frame at timestamp $t$. 

%\subsubsection{Reconstruction}

%The reconstructor recreates the incoming stream of images representing both nominal and (gradually injected) novel unexpected conditions (\autoref{fig:example}). 


\subsection{Usage Scenario}\label{sec:usage-scenario}

\autoref{fig:testing} shows how \tool is used online for misbehaviour prediction after model training (i.e., after fitting the gamma distribution and estimating the threshold $\theta$). Misbehaviour prediction is executed online as the SDC drives. 
In this phase, the SDC generates data continuously and the reconstructor recreates the incoming stream of images. The sequence of reconstruction errors is passed through the autoregressive model $f$ and the resulting, filtered error is compared against the threshold $\theta$, which determines whether an anomaly is detected or not. In the former case, self-healing is triggered and the SDC is brought to a safe state.

\subsubsection{Time-aware Anomaly Score Prediction}\label{sec:time-aware-anomaly-score}

The reconstruction error $e_t$ at time $t$ might be susceptible to single-frame outliers, which are not expected to have a big impact on the driving of the car, but would indeed make the misbehaviour predictor falsely report an anomalous context.
For this reason, we smooth such noisy oscillations by applying an autoregressive filter:
the sequence of reconstruction errors is passed to a module that performs time series-analysis. In \autoref{fig:testing}, this corresponds to the AR filter $f$. The output of this filter, instead of the raw reconstruction error $e_t$, is compared with the threshold $\theta$ to recognize unexpected driving conditions. In our experiments we used a simple AR model (see \autoref{eq:ar}) with $\alpha_0 = 0$ and $\alpha_i = 1/k$ for $i = 1, \ldots, k$.
%Such module analyses the distribution of errors in a window-manner, and determines, within a time window $t_{dec}$, whether the average reconstruction errors in each window correlates with an uncertain driving behaviour. If so, an \textit{alert} is sent either to the self-driving car module or the human driver, to promptly warn of the incoming unsupported driving condition.


%To overcome this problem, an alert is triggerd only if $\mathcal{L}_k(\boldsymbol{x^{i}})$ is bigger than a given threshold,
%where $\mathcal{L}_k(\boldsymbol{x^{i}})$ is a weighted average of the losses over the last $k$ images:
%
%\begin{equation*}
%        \mathcal{L}_k(\boldsymbol{x^{i}}) = \sum_{j \in \{0,\dots,k-1\}} w_j * \mathcal{L}(\boldsymbol{x^{i-j}}, g(f(\boldsymbol{x^{i-j}}))),
%\end{equation*}
%
%where $w_i \in \{w_0,\dots, w_{k-1}\}$ are the weights.
%For simplicity, we use $w_i = \frac{1}{k} \forall i \in \{0,\dots,k-1\}$, and a careful weighting is left for future work.
%


%\subsection{Implementation}\label{sec:implementation}
%
%We implemented our approach in a Python tool called \tool, which is available~\cite{tool}. 
%The tool supports SDC models written in Keras 2.2.4, and has been experimented on the Udacity simulator for self-driving cars~\cite{udacity-simulator}. \andrea{complete if space allows}





==> paper-anomaly-detection copy/5-evaluation.tex <==
% !TEX root =  paper.tex

\section{Empirical Evaluation}\label{sec:evaluation}

\subsection{Research Questions}

We consider the following research questions:

\noindent
\textbf{RQ\textsubscript{1} (effectiveness):}
How effective is \tool in predicting anomalies for autonomous vehicles? What are the best reconstructors to use?

\noindent
\textbf{RQ\textsubscript{2} (prediction):}
How does the misbehaviour predictions of \tool change as we increase the reaction period (i.e., we anticipate the time of prediction)?

\noindent
\textbf{RQ\textsubscript{3} (comparison):}
How does \tool compare with DeepRoad's \cite{deeproad} online input validation?

\subsection{Self Driving Car Models}
We evaluate our framework on three existing DNN-based SDCs: NVIDIA's DAVE-2~\cite{nvidia-dave2}, Epoch~\cite{epoch}, and Chauffeur~\cite{chauffeur}.
We choose these models because they are publicly available, thus they can be trained and evaluated on the simulator. Moreover, they have been objects of study of other testing works~\cite{deepxplore,deeptest}.
DAVE-2 consists of three CNNs, followed by five fully-connected layers. Chauffeur uses a CNN to extract the features of input images, and a RNN to predict the steering angle from 100 previous consecutive images. Epoch consists of a single CNN model.
%DAVE-2 consists of three 5x5 convolutional layers with stride 2 plus two 3x3 convolutional layers, followed by five fully-connected layers with dropout and ReLu activation function. Chauffeur uses a convolutional neural network (CNN) to extract the features of input images, and then utilizes a RNN to predict the steering angle from 100 previous consecutive images. Epoch consists of a single CNN model.

\subsection{Simulation Platform}\label{sec:simulator}

A major problem in anomaly detection research is the lack of labeled benchmark datasets~\cite{Campos:2016:EUO:2962863.2962870}, and the self-driving car domain is no exception.
Unlike previous works~\cite{deeproad,deeptest,deepxplore}, we cannot rely on existing driving image datasets such as the ones released by Udacity~\cite{udacity-datasets}, because they lack any episode of crash, or cars driving off road whatsoever. Moreover, our definition of misbehaviour (\autoref{sec:problem}) requires the creation of a set of ``controllable'' unexpected conditions that may potentially cause them, along with a way to precisely record them.
Thus, to investigate the effectiveness of our approach in predicting safety-critical misbehaviours, we evaluated \tool in the Udacity simulator~\cite{udacity-simulator}.

The Udacity simulator is developed with Unity~\cite{unity}, a popular cross-platform game engine.
The simulator provides two default tracks, %\footnote{https://assetstore.unity.com/packages/3d/environments/roadways/lake-race-track-55908}\textsuperscript{,}\footnote{https://github.com/udacity/self-driving-car-sim/blob/master/Assets/1\_SelfDrivingCar/ Scenes/JungleTrackTraining.unity}
for testing DNNs models. The simulator executes in two modes: (1)~\textit{training mode}, in which the user manually controls the car while the simulator records her actions, and (2)~\textit{autonomous mode}, in which the car is controlled by an external agent, such as a DNN-based autonomous driving system.
Moreover, we added a third track~\cite{mountain-track} to the existing set,
%\footnote{https://assetstore.unity.com/packages/3d/environments/roadways/mountain-race-track-53775}
%
%\head{Lake Track (Track1)} is a simple circuit design with gentle bends, a wide road section, a bridge, and safety tires and road signs. The street is located on the edge of a lake, therefore the car easily falls within the lake if the lane keeping is violated.
%
%\head{Jungle Track (Track2)} is a hard circuit design with highly narrow curves. It is located in the middle of a mountain valley with lots of trees, a smaller road section than Track1, and very limited visibility due to elevation changes.
%
%\head{Mountain Track (Track3)} is a snowy mountain race track having one difficult and narrow curve, many long and soft curves, and a narrow road section. Strong changes in lighting conditions due to tunnels are present, which also block the background view. Finally, concrete barriers placed on street lines create obstacles that need to be avoided.
%
and we implemented two additional components, namely, an \textit{unexpected context generator}, and a \textit{collision/OBE detection system}.

\subsubsection{Unexpected Context Generator}\label{sec:ucg}

First, we developed a method to gradually inject unseen conditions during testing mode (i.e., conditions diverse from the training mode's defaults).
%\head{Day/Night}
The first condition deals with illumination and introduces a \textit{day/night cycle} component to gradually change the light condition of the track during the simulation. The effect is customizable and consists of smooth increase/decrease of brightness/darkness over a fixed period (60~s in our experiments).
%\head{Weather Conditions}
The second kind of unexpected condition deals with \textit{weather}. We implemented rain, snow and mist effects, with a variable intensity during the simulation. For the implementation, we used a specific Unity component called Particle System~\cite{particle-system}
%\footnote{https://docs.unity3d.com/ScriptReference/ParticleSystem.html}
which can simulate the physics of a cluster of particles with high performance. Rain particles emission rate ranges between a minimum of 100 (light rain) to a maximum of 10,000 particles/s (heavy rain); fog between [100..2,000] particles/s, and snow between [100..800] particles/s.
\autoref{fig:effects} shows a few examples.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.3\linewidth]{images/track1_sunrise.pdf}
    \includegraphics[width=0.3\linewidth]{images/track1_fullday.pdf}
    \includegraphics[width=0.3\linewidth]{images/track1_fullnight.pdf}
    \includegraphics[width=0.3\linewidth]{images/track1_snow.pdf}
    \includegraphics[width=0.3\linewidth]{images/track2_mist.pdf}
    \includegraphics[width=0.3\linewidth]{images/track3_rain.pdf}
    \caption{(top) Day/night cycle (sunrise, day, night) and (bottom) weather effects (snowy Lake Track, foggy Jungle Track, and rainy Mountain Track).}
    \label{fig:effects}
\end{figure}

\subsubsection{Collision/OBE Detection System}

Following our definition of safety-critical misbehaviours, we implemented an automated collision/OBE detection system (ACODS) that records any unwanted interaction of the SDC with the environment, allowing us to experiment the effectiveness of \tool at anticipating such episodes during the occurrence of unexpected scenarios (\autoref{sec:ucg}).

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.4\linewidth]{images/simulator_advance_crash_detection.pdf}
    \includegraphics[width=0.4\linewidth]{images/simulator_advance_off_road_detection.pdf}
    \caption{Simulator crash/OBE detection.}
    \label{fig:crash-detection}
\end{figure}

%The output of ACODS is critical in our experimental study, because it is basically the input of \tool \paolo{wrong!}. Therefore it should be designed in a way that is (1)~independent from any specific anomaly detector, and (2)~highly accurate. Therefore, we excluded mathematical formulas based on the position of the car w.r.t. the road which are hard to generalize for all different tracks, and are susceptible of under/over estimations unless careful selection of parameters is used, which is, again, hard to generalize.
We implemented ACODS based on \textit{colliders}, which are consolidated building blocks of modern game engines to simulate the physical interaction between objects. We approximate the car body with a geometry mesh, and implemented a collider callback that informs the simulator of any physical interaction of the car with scene objects. When the car ``hits'' the road, then it means the car is actually on track, whereas when the car ``collides'' with any other object, the callback registers whether it is a crash against some object (\autoref{fig:crash-detection}~(left)), or whether it is an OBE (\autoref{fig:crash-detection}~(right)).

Secondly, we implemented an automatic restart mechanism that restores the SDC to a safe position after a crash/OBE, allowing us to record multiple simulations without the need for manual restart.
%This was implemented leveraging track waypoints, i.e., phantom objects that are used to mark certain positions and directions in a 3D scene. Essentially, each consecutive pair of waypoints $w_n, w_{n+1}$ defines a track sector (which also gives us a way to monitor and control the length of the simulations). Automated restart is performed as follows. If the car crashes at some sector $w_n, w_{n+1}$, we tag the sector as not complete, and the system automatically moves the car to the waypoint $w_{n+1}$, adjusting position and angle according to the waypoint orientation.

\subsection{Procedure}

\subsubsection{Data Generation (Training Set)}\label{sec:data_generation}

Training data were collected by the authors in training mode by performing 10 laps on each track, following two different track orientations (normal, reverse). Overall, we obtained a dataset of 124,638 training images (at 10-13 fps), divided as follows: 32,243 for Track 1 (Lake), 51,422 for Track 2 (Jungle), and 40,973 for Track 3 (Mountain). Differences depend on the track lengths.
To allow a smooth driving and a correct behaviour capture (i.e., lane keeping), the maximum driving speed was set to 30 mph, the default in the Udacity simulator.

\subsubsection{SDC Model Setup \& Training}\label{sec:model-training}

All SDCs models were trained on 41,546 images from the central camera.
We used data augmentation as a consolidated practice for building more reliable and generalizable SDCs, limiting the lack of image diversity in the training data. Specifically, 60\% of the data was augmented through different image transformation techniques (e.g., flipping, translation, shadowing, brightness). We cropped the images to 66 x 200, and converted them from RGB to YUV colour space.
%\paolo{Didn't you use lateral cameras for data augmentation? That's also a consolidated practice.} \andrea{no, we didn't}
All SDC models were trained for 500 epochs with batch size of 256 on a machine featuring an i9 processor, 32 GB of memory, and an Nvidia GPU 2080 TI with 11GB of memory. Basically, the training was meant to create solid models for testing, i.e., able to drive multiple laps on each track under nominal conditions without showing any misbehaviour in terms of crash/OBE.

\subsubsection{Evaluation Set}

To collect the evaluation data, we executed 72 simulations (2 laps each) in autonomous mode (3 SDC x 8 conditions x 3 tracks). As in data generation, the maximum speed was set to 30 mph. Specifically, for each SDC and for each track, we performed 1 simulation in the same normal conditions as the training set. This allows us to estimate the number of false alarms (false positives) in nominal conditions. 
Second, we performed 4 simulations activating in turn a single unexpected condition: day/night cycle, rain, snow, fog. Third, we performed 3 simulations activating in turn a combined condition: day/night cycle + rain, day/night cycle + snow, day/night cycle + fog.

%\begin{itemize}
%    \item First, we performed one (1) simulation on the same normal conditions as the training set. This allows us to estimate the number of FP.
%    \item Second, we performed four (4) simulations activating in turn a single unexpected condition: day/night cycle, rain, snow, fog.
%    \item Third, we performed three (3) simulations activating in turn a combined unexpected condition: day/night cycle + rain, day/night cycle + snow, day/night cycle + fog.
%\end{itemize}

In our experiments, we used a value of 60~s both for the day/night cycle and for the loop between the minimum and maximum intensity of the effects. This value was chosen empirically given the relatively short speed of the SDC, and the small length of the tracks, and allowed us to test the behaviour of the SDC on each of the track subsets under all possible conditions. For example, the bridge part of Track1 (Lake) has been driven on under both dawn/day/sunset/night conditions (day/night cycle) and minimal/maximal intensity of rain/fog/snow.

Overall, we obtained a dataset of 778,592 images, divided as follows: 188,032 for Track 1 (Lake), 260,064 for Track 2 (Jungle), and 208,064 for Track 3 (Mountain) with unknown conditions and 33,088 for Track 1, 46,272 for Track 2 and 43,072 for Track 3 in known conditions.


\begin{figure*}[t]
    \centering
    %TODO Graphics Sizing
    \includegraphics[scale=0.8]{images/window-labelling.png}
    \caption{Labelling of Anomalous and Normal Windows in Driving Stream.}
    \label{fig:labelling}
\end{figure*}


\subsubsection{\tool's Configurations}

%\head{Variants Setup \& Training}
We used four autoencoders taken from existing guidelines~\cite{keras-autoencoders}: %with some minor changes:
(1)~\emph{SAE} (simple autoencoder with a single hidden layer),
%$\boldsymbol{Z} = 64$ and ReLu activation function.
(2)~\emph{DAE} (deep five layers fully-connected autoencoder),
(3)~\emph{CAE} (convolutional autoencoder alternating convolutional and max-pooling layers), and
(4)~\emph{VAE (variational autoencoder)}.

All autoencoders take as input a single image. We added images taken by the side cameras of the car (left, right) to allow better generalization, even though, during testing, autoencoders are not used for prediction. Lastly, we performed further data augmentation on 60\% of the inputs, as described in \autoref{sec:model-training}.

As an additional sequence-based reconstructor, we also implemented an LSTM consisting of two LSTM-layers and one convolutional layer.
%
%The last considered anomaly detector consists in a Long Short Term Memory (LSTM) consisting of two LSTM-layers and one convolutional layer.
%More in detail, at time $t$, LSTM takes as input a sequence of images $<\boldsymbol{x^{t-15*15}}, \boldsymbol{x^{t-14*15}}, \dots, \boldsymbol{x^{t-1*15}}>$ which is used to predict the current image $\boldsymbol{x^{t}}$.
%All considered reconstructors were trained to minimize the MSE between the predicted image and the observed one.
For implementation details, we made our code publicly available in the replication package accompanying this paper~\cite{tool}.

%We implemented and trained five neural networks to serve as anomaly detectors in our simulations:
%First, we use four autoencoders (see \autoref{sec:autoencoders}) taken from the \emph{Building Autoencoders in Keras Tutorial}~\cite{keras-autoencoders} with some minor changes:
%A \emph{simple autoencoder (sae)} with a single dense hidden layer,
%a \emph{deep fully-connected autoencoder (dae)}, consisting of five dense hidden layers,
%a \emph{convolutional autoencoder (cae)}, particularly designed to capture features of images
%and a \emph{variational autoencoder (vae)}, a somewhat more novel and sophisticated model, as explained in\cite{keras-autoencoders}.
%All autoencoders take as input a single image.
%As they are computationally very efficient, we added images taken by the side cameras of the car to the train set.
%While in the evaluation of \tool the autoencoders never have to predict such side camera images, training with them still allows the neural network to generalize better.
%Lastly, we perform some simple data augmentation on 60\% of the autoencoders inputs.

%Second, we implement a simple LSTM, as explained in section \autoref{sec:rnn}, consisting of two lstm-layers and one convolutional layer.
%At time $t$ takes as input a series of images $<\boldsymbol{x^{t-15*15}}, \boldsymbol{x^{t-14*15}}, \dots, \boldsymbol{x^{t-1*15}}>$ and is trained to predict $\boldsymbol{x^{t}}$.
%Similar to autoencoders, we calculate the novelty prediction by comparing the predicted image to the observed one.
%For implementation details, we refer to our code which is made open source in the replication package accompanying this paper~\cite{tool}.


\head{Baseline}
We use the input validation technique of \deeproad~\cite{deeproad} as baseline for \tool. % and use it in \tool like any of the 5 neural networks explained above.
Unfortunately, authors did not make their code available; therefore, we implemented of our own version according to the description in the paper.
For input validation, \deeproad uses the pre-trained VGG19 ImageNet classifier~\cite{Simonyan2014} to extract style and feature vectors from a given image. Principal Component Analysis (PCA) is then used to reduce all style and feature vectors, concatenated into a matrix, to three dimensional representations, which support distance/similarity estimation.
To allow a fair comparison, we integrated it within \tool as reconstructor. However, unlike autoencoders, \deeproad is computationally very expensive and memory demanding (due to the size of the matrix supplied to PCA). In the paper, authors reduced their training set to 600 images, which were resized to 120x90. During input validation, the three dimensional representation of an online input image is compared to the nominal images by measuring the average of the top-100 minimum distances from the training set.

%Even though DeepRoad's high memory requirements are a serious shortcoming, we relaxed the restrictions listed above to allow fair comparison with our computationally less expensive misbehaviour predictor \tool:
% \andrea{I would not draw such conclusions, it's the job of the reviewers}
Our own implementation relaxed the restrictions above by considering a training set consisting of 3,000 randomly sampled images (i.e., $5\times$ improvement w.r.t. the original implementation described in the paper), resized to 224x224, which is the default input size for VGG19~\cite{keras-vgg19}. Keeping the fraction of the training set ($\frac{1}{6}$) constant, we compute similarity based on the average of the top-500 minimal distances.
For implementation details, we made our code publicly available in the replication package accompanying this paper~\cite{tool}.
%We further use the VGG19 weights provided by Keras~\cite{keras-vgg19} for  feature extraction and the PCA implementation available in Scikit-learn~\cite{scikit-svm} for  dimensionality reduction.

%to allow a fairer comparison to our computationally less expensive anomaly detectors:
%(1) We resize the images to $224 * 224$ (default input size for VGG, see\cite{keras-vgg19})
%and (2) we use a training set consisting of 3000 randomly samples images.
%Keeping the fraction of $\frac{1}{6}$ of the training set constant, we compute similarity based on the average of the Top-500 minimal distances.
%We further use the VGG19 weights provided by keras\cite{keras-vgg19} for the feature extraction and the SVM implemented in scikit-learn\cite{scikit-svm} for the dimensionality reduction.

\subsection{Evaluation of Simulation Results}

%We ran our evaluations based on recordings of a SDC, driving on tracks with weather and illumination conditions the car was not trained on.
%\andrea{this is explained later, we need to move this sec in the procedure after Sec 5.6.3 or Sec 5.6.4} \paolo{not sure: it flows well here as well}
To allow a fair comparison with our baseline \deeproad, we evaluated all approaches offline, by splitting the evaluation set of recorded images in \emph{windows of consecutive frames}, which we labelled as either anomalous or normal (\autoref{fig:labelling}).
In anomalous windows, \tool is expected to predict the shortly-following misbehavior. % whereas in normal windows no subsequent misbehavior was recorded.

\subsubsection{Labelling of Anomaly and Normal Windows in Evaluation Data}\label{sec:labelling}

Let $\boldsymbol{X} = \{x_1, x_2, \ldots, x_n \}$ be the sequence of considered images (frames).
Misbehaviors are represented as $m_j \in \{0,1\}$, where $m_j = 1$ iff a misbehavior is recorded at $x_j \in \boldsymbol{X}$.
We define a healing period as a sequence of $h$ misbehaviour-free frames following a misbehaviour at time $t$.
We define a reaction period as a sequence of $r$ misbehaviour-free frames preceding a misbehaviour at time $t'$ and not intersecting any healing period.
We define an \textit{anomalous window} as $a$ consecutive misbehaviour-free frames followed by a reaction period that does not intersect any healing period.
We define a \textit{normal window} as $b$ consecutive misbehaviour-free frames followed by an anomalous window, or a normal window that does not intersect any healing period.
This is illustrated graphically in \autoref{fig:labelling}. Formally, assuming any misbehavior recorded at time $t \in [1{:}n]$, i.e., $m_t = 1$:

\begin{itemize}
    \item window $x_{t+1}$ to $x_{t+h}$ is labelled as healing period if $m_t = 1$ and $m_j = 0 \: \forall j \in [t+1 {:} t+h]$;
    \item furthermore, the window $x_{t+1}$ to $x_{k-1}$ is also labelled as healing period if $m_k = 1$ with $k > t$ and $k-t-1 < h$, and $m_j = 0 \: \forall j \in [t+1 {:} k-1]$;
    \item window $x_{t-r}$ to $x_{t-1}$ is labelled as reaction period iff $m_t = 1$, $m_j = 0 \: \forall j \in [t-r {:} t-1]$ and no healing period contains any frame from $x_{t-r}$ to $x_{t-1}$;
    \item window $x_{i}$ to $x_{i+a-1}$ is labelled as anomaly window iff a reaction period starts at $x_{i+a}$, $m_j = 0 \: \forall j \in [i {:} i+a-1]$ and no healing period contains any frame from $x_{i}$ to $x_{i+a-1}$;
    \item window $x_{i}$ to $x_{i+b-1}$ is labelled as normal window iff an anomaly or a normal window starts at $x_{i+b}$, $m_j = 0 \: \forall j \in [i {:} i+b-1]$ and no healing period contains any frame from $x_{i}$ to $x_{i+b-1}$.
\end{itemize}

Moreover, if $m_j = 0$ for all $j \in [k{:}n]$, all consecutive windows of size $b$ starting within $x_{k}$ to $x_{n-r-a-1}$ which do not intersect any healing period are labelled as normal.
%Assuming any misbehavior recorded at time $t \in [1{:}n]$, i.e., $m_t = 1$, anomaly and normal windows are defined as follows:
%\begin{itemize}
%    \item window $x_{t-r-a}$ to $x_{t-r-1}$ is labelled as anomaly window iff $m_j = 0 \: \forall j \in \mathbb{N}_s: t-r-a-h \leq j \leq t-1$;
%    \item windows $\boldsymbol{x}^{t-r-a-p*n}$ to $\boldsymbol{x}^{t-r-a-(p-1)n-1}$ are labelled as normal window for each $p \in \mathbb{N}$ where $m_j = 0 \: \forall j \in \mathbb{N}_s: t-r-a-h-(p*n) \leq j \leq t-1$
%\end{itemize}
%, where $r \in \mathbb{N} $ and $h \in \mathbb{N}$ are constants.
The labelling described above ensures that after the last misbehavior in a sequence, $h$ \emph{healing images} are ignored (i.e., not labeled) before another anomaly or normal window is defined.
$h$ must be chosen high enough that the car is back safely on the road when the next windows are labelled.
Furthermore, $r$ images occur in between an anomaly window in which the system is supposed to predict the upcoming misbehavior, and the actual misbehavior.
This period would, in practice, be used by the self-healing system to execute countermeasures against the predicted future misbehavior.
Intuitively, misbehavior prediction is expected to be much harder as the value of $r$ increases. In our experiments, we set the value of $n = b = 30$ frames (i.e., normal/anomalous windows), which is $\approx$3s.\footnote{In our setting, Udacity frame rate was approximately 10/12 fps.} The size of the healing window was set to $h = 60$ (> 5s) frames, and the size of the reaction window to $r = 50$ (> 4s) frames.

\subsubsection{Metrics used for Analysis}\label{sec:metrics_analysis}

If the loss score for an image is higher than the automatically estimated threshold $\theta$ (\autoref{sec:usage-scenario}), \tool triggers an alarm.
Consequently, a true positive is defined when \tool triggers an alarm during an anomalous window, early enough to predict a misbehavior. Conversely, a false negative occurs when \tool does not trigger an alarm during an anomalous window, thus failing at predicting a mis-behaviour in time for triggering self-healing.
A false positive represents a false alarm by \tool, whereas true negative cases occur when \tool detects correct detection of normality.

%Ideally, an alarm is raised at least for one input image in an anomalous window (thus predicting a misbehavior) and
%never in a normal window (thus not raising any false alarms).
%Accordingly, we define the following metrics:

%\andrea{I agree it is intuitive; I tried compress it, let's see if space allows saving it}
%\paolo{Everybody knows TP, FN, FP, TN, so if we need space we can drop the following definitions. We may just briefly say that based on our definitions of anomaly/normal windows, we can measure TP, FN, FP, TN from the  confidence estimated as the car runs.}
%\begin{description}
%
%    \item[true positive (TP)] An anomalous window is a TP, iff \tool triggers an alarm during an anomalous window.
%    In practice, this means that the self healing system is triggered early enough to prevent a misbehavior.
%
%    \item[false negative (FN)]  An anomalous window is a FN, iff \tool does not trigger an alarm during an anomalous window.
%    In practice, this will lead to an unpredicted misbehavior.
%
%    \item[false positive (FP)] A normal window is a FP, iff \tool triggers an alarm in a normal window.
%    In practice, this will trigger the self healing system in a case where this is not required.
%
%    \item[true negative (TN)] A normal window is a TN, iff \tool behaves correctly by not triggering any alarm in a normal window.
%
%\end{description}

%Note that technically, every single image in a window can cause \tool to trigger an alarm.
We assume that a single alarm immediately starts the self healing system, such that multiple consecutive alarms within the healing time have no  effect.
%Thus, it's possible that a window is TP or FP even if the majority of its images would not trigger an alarm.
Correspondingly, once a FP occurs and the self healing system is running, additional consecutive FP windows have no effect in practice and are thus excluded from our analysis.
%Consecutive TP are impossible by design due to the recovery and reaction periods (see \autoref{sec:labelling}).
%\michael{@paolo, andrea: I think now we are not mentioning anymore that we count consecutive FP only once, even though this has a huge impact on the numbers.}

Our goal is to achieve (1)~high recall, or true positive rate (TPR, defined as TP/TP+FN), i.e., true alarms, while (2)~minimizing the complement of specificity, or false positive rate (FPR, defined as FP/TN+FP), i.e., labelling safe situations as unsafe.
We are also interested in F1-score ($F_{1}=2 \cdot \frac{\text{Precision} \times \text{Recall}}{\text{Precision} + \text{Recall}}$) because, in practice, it is informative to have a high F1-score at a given threshold.
%Moreover, we calculate AUC-ROC, the area under the curve (AUC) of the receiver operating characteristics curve (ROC), created by plotting the TPR against the FPR given all possible thresholds.
%Calculating the AUC-ROC is standard in anomaly detector research \michael{TODO: References}, however, it is not ideal when the evaluation data is heavily unbalanced.

We also consider two widely adopted threshold-independent metrics for evaluating classifiers at various thresholds settings such as AUC-ROC (area under the curve of the Receiver Operating Characteristics), and AUC-PRC (area under the Precision-Recall curve).
%However, AUC-ROC may be not indicative when data are heavily unbalanced, which is our case, since anomalies are rare.
%In such cases, the AUC of the Precision-Recall Curve (PRC) graph is more suitable\cite{PR-ROC, saito_prc_vs_roc}.
%The latter is the case in our setting.
%However, for completeness, we also include AUC-ROC in our analysis.
%\michael{@paolo I know that we agreed to exclude AUC-ROC. However, I wasn't quite sure how to do that without making it look like we're avoiding the AUC-ROC analysis, which is why i (temporarily?) still include AUC-ROC. }
%\paolo{We can include AUC-ROC, but just to show that it is not very informative.}
%\andrea{I would use this insight after we have shown the results. Otherwise it sounds that we are deliberately putting some garbage in the paper, which is an easy hook for revs}


\subsection{Results}

% Note: use the queries in the \images\result-table-query.sql file to extract the numbers for this table
% I generated the table using https://www.tablesgenerator.com/# and you can easily open and edit
% the table there (file -> load table) using the  \images\results-table.tgn file

\input{table-results-95-99}
%\input{table-results-99-999}
%\input{table-results-old}


\head{Effectiveness (RQ\textsubscript{1})}
\autoref{tab:big_results_table} presents the effectiveness results on a per-SDC model basis. Columns~2 and~3 show threshold-independent measures of AUC-PRC and AUC-ROC. The remaining of the table shows the effectiveness metrics across two confidence thresholds that we found interesting for analysis and correspond to $\epsilon = 0.05$ and $\epsilon = 0.01$ (at lower values of $\epsilon$, both FPR and TPR get close to zero, making the misbehaviour predictor useless).

Overall, LSTM and VAE are the best performing reconstructors on the AUC-PRC and AUC-ROC metrics.
%While values of AUC-ROC suggest an overall good prediction score by all techniques, this result may be not indicative because our data are heavily unbalanced towards anomalous conditions.
%We find that our anomaly detectors are very effective at predicting misbehaviors.\footnote{Please note that we will not discuss the performance of our benchmark, deeproad in RQ\textsubscript{1}, but do so in detail in the discussion RQ\textsubscript{3}}.
%With a threshold based on confidence interval of 0.99, SAE performed similar to the VAE with the 0.999 based threshold, which is an interesting finding given its very simple design.
%At a threshold based on a 0.999 confidence interval, the best performing anomaly detector is VAE, predicting \hl{more than half (112} out of \hl{218}) misbehaviors.
%At the same time, VAE only triggers \hl{191} false alarms (FPR \hl{0.06}).
%Note that these false alarm were raised during testing, with increasingly novel driving conditions (i.e., light snow/rain). Thus, a generally low confidence in the SDC behaviour is expected even if we no misbehaviours were observed. %Hence, a risk averse car owner may not consider these alarms as false positive.
Columns~12 and~21 (Nominal/FPR) show  FPR under conditions similar to those of the training set. Values are almost always near to zero and occasionally even equal to zero (this is indicated by omitting the decimals) across the variants of \tool. This is an empirical validation of the accuracy of the gamma distribution as a statistical model for the reconstruction errors. In fact, at $\epsilon = 0.05$ most FPR reported in column 12 are very close to the theoretical value, 0.05 (see, e.g., rows under \textit{Totals}). At $\epsilon = 0.01$ some values drop to zero. This means that in those configurations \tool will raise no false alarm when the SDC drives in nominal conditions.
%This is essentially a sanity check that all SDCs are highly reliable in (self-)driving on nominal conditions, and no false alarms are raised by \tool.
For instance, with both thresholds, LSTM never raised false alarms within the 23,728 considered normal windows .
%On the other hand, FPR of \deeproad is always non negative even under normal conditions (3-4\% false alarms).

%To test the FPR under conditions known to the cars, we repeated the experiment under known conditions. With the same threshold, VAE \hl{not falsely alert once} within \hl{1561} considered normal windows (gray column in \autoref{tab:big_results_table}).

In terms of TPR (to be maximized) and FPR (to be minimized), the best reconstructors are VAE and SAE, with comparable overall performance: 
 77\%, 11\% (TPR, FPR of VAE) and 72\%, 10\% (SAE) at $\epsilon = 0.05$; 55\%, 5\% (VAE)  and 59\%, 5\% (SAE) at $\epsilon = 0.01$.
It can be noticed that FPR is higher than $\epsilon$ (10\% vs 5\% and 5\% vs 1\%) with both reconstructors. This is expected, since we are measuring FPR in tracks with injected anomalies. These tracks differ substantially from the nominal tracks even in conditions not so extreme as to cause a misbehaviour, hence inflating the FPR a bit. However, we can notice that even in such non nominal conditions, the FPR remains low and not too far from the theoretical prediction $\epsilon$.
%The TPR of dae, cae and lstm is still very low with a threshold based on confidence interval of 0.99 but increases notably with a decreasing threshold.
%In fact, looking at the threshold independent AUC-PRC and AUC-ROC, lstm and dae are comparable to vae and sae, with the cae only slightly behind.

%It is worth mentioning that the goal of this paper is not to compare various autoencoder techniques and lstms, but rather to show that even implementations which are intentionally kept simple can provide very effective misbehavior predictions for SDC.

%For further analysis of the effectiveness of our anomaly detectors, we refer to \autoref{tab:big_results_table}

We can \textbf{answer to RQ1} by noticing that with reconstructors VAE and SAE we achieve a FPR in nominal conditions close to the theoretical expectations (resp. 5\% and 1\%, in the two considered configurations); that in anomalous conditions FPR increases by a moderate amount (resp., +5\% and +4\%); and that the achieved TPR is quite high (with VAE, SAE, resp. 77\%, 72\% and 55\%, 59\%).

\head{Prediction (RQ\textsubscript{2})}
\autoref{fig:prc_reaction} shows the PRC-AUC of the various configurations of \tool over different reaction periods.
The general trend is that predictions get harder when the SDC is far from a critical scenario, having a longer reaction period to prevent the misbehavior, but quite surprisingly there is no drop in performance as we move away from the misbehaviour. Our explanation of this unexpected finding is that the tracks used for the evaluation of the approach contain always a relatively high degree of anomalous features, which might trigger a self-healing reaction. Occasionally, the level of detected anomalies  surpasses the threshold and the misbehaviour predictor raises an alarm. Correspondingly, although slightly reduced,  the signals of an upcoming misbehaviour exist in images quite far (even 60 frames or around 6s) from the misbehaviour. 

We can \textbf{answer to RQ2} by noticing that the performance of \tool degrades smoothly as we anticipate the prediction (AUC-PRC remains quite high even 6s before the misbehaviour), but we should also remark that this result must be taken with care and might be partially due to the characteristics of the considered tracks, which contain a continuously and smoothly increasing degree of injected anomalies by design.

%However, even for 100 frames (> 8s) ahead of the misbehavior, the values for PRC-AUCS are still clearly better than those of a random classifier,\footnote{The expected AUC-PRC of a random anomaly detector is A / (A + N), where A is the number of anomalous and N the number of normal windows~\cite{saito_prc_vs_roc}.} which indicates that \tool is capable of predicting a large number of unexpected execution contexts that subsequently cause a misbehavior.

%\michael{I don't really know what else to say here. Suggestions? My try:}
%It is particularly interesting to observe the fact that LSTM is very efficient for short reaction periods, probably due to its retrospectively capability of processing historical information. In practice, the short-notice prediction capability of LSTM may be leveraged to create an ensemble of redundant predictors, that compensate for each other weaknesses.
% proof very useful in combination with other anomaly detectors to take over if they have failed.
%For instance, should the VAE fail at predicting a hazardous situation before the reaction period failed, SDC could still trigger some last-second self healing mechanism thanks to LSTM (e.g., studies on pre-crash automated seat belt systems~\cite{doi:10.1177/1687814017725246,Lee2013StudyOE} confirmed a [-3s..-0.5s] as reaction period for activation of actuators for tightening seat belts).
%(tighten seat belts) .

\head{Comparison (RQ\textsubscript{3})}
%Both models outperform \deeproad over all metrics.
%In terms of AUC-ROC, all variants of \tool obtain high prediction scores, and outperform \deeproad. The greatest increase is by VAE (+15\%), whereas the smallest is by CAE (+8\%). The best reconstructor is VAE (0.924), with an AUC-ROC increase of 15\%.
%
%A closer look at the other metrics suggest instead a wide gap in prediction capability between \tool and \deeproad.
%In terms of TPR, \tool (SAE) is +186\% effective at predicting misbehaviours than \deeproad, which is indeed an interesting finding given its very simple design.
%
In our experiments, \tool is constantly superior to \deeproad at predicting misbehaviours. Results of AUC-PRC and AUC-ROC show significant improvements across all thresholds, and regardless of the technique being used and the reaction period considered (in \autoref{fig:prc_reaction}, \deeproad is the lowest curve).
With $\epsilon = 0.05$ (resp. $\epsilon = 0.01$), 
VAE and SAE (see \autoref{tab:big_results_table}) expose more than twice the misbehaviours exposed by \deeproad, with a TPR =  77\%, 72\% vs 32\% (resp., 55\%, 59\% vs 20\%), at comparable false positive rate FPR = 11\%, 10\% vs 9\% (resp., 5\% vs 6\%).
%For 0.99 and 0.999 confidence interval based thresholds, VAE and SAE strictly dominate \deeproad in terms of TPR, F1 and precision.
%The only metric where \deeproad has a marginal gain over \tool (VAE) is FPR under novel conditions in the 0.99 context. Nonetheless, in known conditions,
%\deeproad constantly produces more false alarms than any of variant of \tool.

While reimplementing \deeproad, we noticed  its high computational cost that makes it quite unsuitable for online misbehaviour prediction.
SDC manufacturers use much larger training datasets than the one we used for our empirical study and differently from autoencoders such as VAE and SAE, \deeproad is quite sensitive to the size of the training set, which must be sub-sampled dramatically to make the approach applicable. On the contrary, autoencoders seem a very promising option, given their relatively simple architecture. In particular, SAE is very efficient, yet it has comparable performance as the more sophisticated VAE.
Hence, as an input validation framework, \deeproad has shown to be both computationally very expensive and inaccurate, which makes it less promising and desirable than \tool for online misbehaviour prediction.
%Unlike what is stated in the original paper, in our experiments, \deeproad has shown computationally very expensive, as well as highly inaccurate. Thus, we conclude that it is prohibitive thinking about an eventual adoption in the field of online misbehaviour prediction.
%This makes it less useful in practice.
%As a comparison: The stored SVM used for deeproad in our experiments requires 11.9GB when stored on the file system - our best performing vae and sae only require 450MB and 56.7 MB, respectively.

Our \textbf{answer to RQ3} is that \tool outperforms \deeproad in all respects: computational cost, accuracy of misbehaviour prediction (see TPR) and minimization of false alarms (see FPR and AUC-PRC).

\begin{figure}[t]
    %TODO Graphics Sizing
    \includegraphics[scale=0.25]{images/AUC-PRC-reaction-time-an30_h60_k4.png}
    \caption{Misbehavior prediction capability over time.}
    \label{fig:prc_reaction}
\end{figure}

\subsection{Threats to Validity}\label{sec:ttv}

\head{Internal validity}
We compared all variants of \tool and \deeproad under identical parameter settings, and on the same evaluation set.
The main threat to internal validity concerns our custom implementation of unexpected conditions within the simulator. However, this was a mandatory choice, since we are not aware of open source driving simulators that can inject unexpected execution contexts in a controllable way. 
Another possible threat may be the choice and the training of our own SDCs, which may exhibit a large number of misbehaviour if trained inadequately. 
We mitigated this threat by training and fine-tuning the best publicly available driving models. Our own implementation of \deeproad may be another threat to internal validity, that we mitigated by developing an implementation which improves the original one by processing $5\times$ more information.

\head{External validity}
We used a limited number of self-driving systems in our evaluation, as well as tracks, which pose a threat in terms of generalizability of our results. We tried to mitigate this threat by choosing popular subjects developed with real-world frameworks (e..g, Keras). % and trained  quite strong SDC. %However more subject systems are needed to fully address the generalization threat.

\head{Reproducibility} 
All our results, the source code of \tool, the simulator, and all subjects are available~\cite{tool}, making the evaluation repeatable and our results reproducible.


==> paper-anomaly-detection copy/6-discussion.tex <==
% !TEX root =  paper.tex
\section{Discussion}\label{sec:discussion} 

\begin{itemize}
\item What are the limits of our techniques, what mis-behaviour we were unable to detect? Was it the time to detection too short?
\end{itemize}


==> paper-anomaly-detection copy/7-related.tex <==
\section{Related Work}\label{sec:relwork}

%To the best of our knowledge, our paper is the first to propose an approach for the prediction of misbehaviours in DNN-based systems due to unexpected driving conditions, with the intent of enabling self-healing procedures. As such, the only related works that are directly comparable to ours are those performing input validation and anomaly detection. 
%However, since we want to recognize such critical scenarios if they are not represented, or underrepresented in the training set, for completeness we report also a summary of the literature on DNN test generation. 

\head{Adversarial Input Generation}
%\subsubsection{Adversarial Generation}
Adversarial generation approaches aim at generating inputs that trigger inconsistencies between multiple autonomous driving systems~\cite{deepxplore}, or between the original and transformed driving scenarios~\cite{deeptest,deeproad,7313519}. %Such frameworks alter the input images fed to the DNN by means of artificial transformations (e.g., lightning effects and occlusions~\cite{deepxplore}, affine transformations~\cite{deeptest}), as well as generative adversarial networks~\cite{deeproad}, to simulate adversarial driving conditions.
%
%For example, a number of 
%M\"{u}ller et al.~\cite{7313519}
%DeepExplore~\cite{deepxplore}, DeepTest~\cite{deeptest} and DeepRoad~\cite{deeproad} test the robustness of self-driving car modules. % from Udacity self-driving car challenge. 
%In these papers, the proposed frameworks synthesize alternative driving images simulating adversarial driving conditions. %DeepExplore~\cite{deepxplore} uses lightning effects and occlusions to transform the testing data into artificially simulated adversarial inputs. DeepTest~\cite{deeptest} alters the images using synthetic affine transformation from the computer vision domain, such as blurring and brightness adjustments, and Photoshop to create simulated rain/fog effects. Differently, DeepRoad~\cite{deeproad} generates images by means of Generative Adversarial Networks (GANs). 
%Generated images are then validated by measuring their distance in the latent space produced by PCA with respect to the training images. 
%Results show that anomalies created in this way have larger mean squared error (MSE), therefore in many cases they fool the DNN that predicts the steering angle. 
%
These works exploit the well-known fragility of DNNs to adversarial examples. Therefore, their main use-case concerns the identification of underrepresented scenarios in the training data (e.g., snowy weather condition) to support re-training and better generalization after re-training. 
The only comparable technique is the online input validation of \deeproad~\cite{deeproad}, for which we carried out an explicit comparison in our empirical study, finding poor performance when used for online misbehaviour prediction.

% proposes also an interesting approach in which input images are validated by measuring their distance in the latent space produced by PCA with respect to the training images. When the latent space distance of an input image is higher than a given threshold, the input is deemed invalid. In principle such an approach could be used also for online misbehaviour prediction (an invalid input may be considered as an input possibly leading to a misbehaviour). Thus, we carried out an explicit comparison with \deeproad in our empirical study (\autoref{sec:evaluation}).

%Indeed, results have shown that such adversarial inputs are easily avoided by retraining the DNN.

%Paolo: I do not think we can compare their threshold (which is actually an approximation of the functional oracle) with our threshold (used to perform anomaly detection): they approximate bug detection with inconsistency above threshold and they need such approximation to know if the generated test cases are useful or not; we do not use the threshold to evaluate any test case, because we do not generate test cases (we detect anomalies)
%In these works, essentially, any deviation from the nominal data distribution according to a given threshold is considered as a potential car crash, and authors claim that such ``crashes'' will be avoided by using such frameworks.
%However, single steering angle mis-predictions for \textit{individual} recorded images are not guaranteed to actually lead to car accidents, since other variables (e.g., speed, entrance angle in a curve) need to be taken into account. More importantly, driving images datasets used in such papers do not contain any crash or OBE whatsoever. 
 
%Thus, existing works claim that crashes would have been avoided by using their frameworks, but they actually never experimented it on real driving simulator,
%Second, even if the car is driving in an adversarial situation, it is not clear whether the controlling system would have enough time to react (or to warn the driver). Thus, existing works claim that crashes would have been avoided by using their frameworks, but they actually never experimented it on real driving simulator, in which crashes can be objectively identified. 

%In an online context, such approaches are not expected to work well, as anomalies do not consists of individual images, but rather of a sequence of images representing a challenging driving scenario that gradually lower the confidence of the DNN leading to an observable misbehaviour. \andrea{to be verified!}
%\andrea{the msg here is that, even if a single prediction is wrong, it is not said that the car would crash}

%Similarly to these works, we test the self-driving car against adversarial conditions represented by unseen weather conditions. Differently, in this paper we tackle the problem of \textit{online testing} of autonomous driving systems, by proposing a runtime anomaly detection system to predict the occurrence of misbehaviours due to unseen environmental conditions at runtime. 

Despite the different goal (test generation vs misbehaviour prediction), we share with these works the problem of how to empirically validate the proposed technique in the absence of a precise oracle that defines the expected behaviour of a self-driving car. The prevalent choice in test generators~\cite{deeptest,deeproad,7313519,deepxplore} is to address the oracle problem by \textit{differential testing}, i.e., by comparing the behaviours of multiple DNNs, or by \textit{metamorphic testing}, i.e., by comparing the behaviour before and after applying a metamorphic transformation to the input. Approaches based on verification are also being under investigation~\cite{deepsafe}.
In this paper, we adopt a precise definition of \textit{DNN misbehaviour}, which gives us a very accurate \textit{functional oracle}, with no need for differential testing, metamorphic testing, or verification. 

%DeepSafe~\cite{deepsafe} uses verification to assess the overall robustness of a neural network against adversarial examples. In particular, it applies clustering over labeled data and it leverages constraint solvers to automatically identify safe regions in which the network is robust. DeepSafe can guarantee that all the inputs in safe regions are classified correctly and it can generate adversarial examples for the unsafe regions.


\head{Search-based Generation}
Abdessalem et al.~\cite{Abdessalem-ASE18-1,Abdessalem-ASE18-2,Abdessalem-ICSE18} combine genetic algorithms and machine learning  to test a pedestrian detection system. 
Mullins et al.~\cite{MULLINS2018197} use Gaussian processes to drive the search towards yet unexplored regions of the input space, whereas Gambi et al.~\cite{Gambi:2019:ATS:3293882.3330566} propose \textsc{AsFault}, a search-based test generator for autonomous vehicles based on procedural content generation. 
\textsc{AsFault} uses search operators which mutate and recombine road segments to construct road networks for testing the lane keeping functionality of self-driving cars. Their goal is to generate extreme and challenging roads, maximizing the number of observed OBEs, while our goal is to avoid OBEs by predicting misbehaviours.

%\subsubsection{Adequacy Criteria}
%DeepExplore~\cite{deepxplore} introduces neuron coverage as adequacy criterion for systematically measuring the parts of a deep learning system exercised by the test inputs.
%On the same line, Kim et al.~\cite{Kim:2019:GDL:3339505.3339634} propose several white-box test adequacy criteria based on surprise, defined as the distance in DNN's behaviour between a new, candidate test input and the training data. Inputs should be generated to cover all ranges of surprise, from low to high surprise.
%DeepGauge~\cite{Ma:2018:DMT:3238147.3238202} present a set of multi-granularity testing criteria for DNNs that support finer grain assessment than neuron coverage~\cite{deepxplore}. In another work, Ma et al.~\cite{8668044} reformulate traditional combinatorial testing using the neuron activation values as parameters. 
%Differently, our approach aims at recognizing unexpected conditions, not at generating adequately covering test inputs. 
%We assume that our approach is applied after adequacy criteria have been employed to augment the training set as much as possible, aiming for the online identification of the residual misbehaviours of the system.


\head{Anomaly Detection for Time Series}
Anomaly detection for self-driving vehicles has been studied from a security perspective. For example, Narayanan et al.~\cite{Narayanan} use a Hidden Markov Model to detect malicious behaviours from real vehicles, and issue alerts while a vehicle is in operation. Taylor et al.~\cite{7796898} use LSTM neural networks to detect car's controller area network (CAN) bus attacks, whereas Marchetti et al.~\cite{7740627} used an information theoretic approach.
Lin et al.~\cite{5509781} used the Mahalanobis distance between multiple sensor data to identify unusual events in Unmanned Aerial Vehicles (UAVs). However, their approach is not image-based and thus is not comparable with our work.
Moreover, ours is the first approach that detects unexpected driving conditions for the prediction of misbehaviours of an autonomous vehicle to enable self-healing.





==> paper-anomaly-detection copy/8-conclusion.tex <==
% !TEX root =  paper.tex
\section{Conclusions and Future Work}\label{sec:conclusions}

In this paper, we studied the problem of estimating the confidence of the DNN-based autonomous in response to unexpected execution contexts.  
Our tool \tool was able to anticipate by several seconds many potentially safety-critical misbehaviours, such as out of bound episodes or collisions, with a low false alarm rate, outperforming the input validator of \deeproad. 
Future work concerns devising novel metrics of DNN confidence, including white-box ones, with a potential for hybridization. 
%Moreover, our autoencoder-based techniques can be combined with advanced image semantic segmentation techniques that provide a context model (scene semantic segmentation) that may help explain how the model behaves.
It would be also interesting to characterize and predict other kind of misbehaviours (e.g., derivative of steering angle) as well as implementing confidence-guided self-healing within the simulator.
We believe that our promising results in online misbehaviour detection, united with the availability of a labeled dataset of crashes and a simulation environment, can foster novel approaches for online prediction and self-healing of autonomous driving systems.

%\begin{itemize}
%\item Uncertainty/Entropy
%\item Optical flow ConvNets
%\item Image Semantic Segmentation. Attention model or scene semantic segmentation could be added. It helps to explain how the model works.
%\item Investigate Model Predictive Control (MPC) for autonomous vehicles. MPC determines a vehicle trajectory with the lowest cost relative to the reference trajectory (waypoints) using an optimizer.
%\item predicting/correcting other signals other than the steering angle (e.g., speed, brake)
%\end{itemize}

%\begin{itemize}
%\item No severity of the anomalies
%\item No other kind of anomalies (derivative of steering angle) which CommaAI models seem to suffer the most
%\end{itemize}

==> paper-anomaly-detection copy/table-results-95-99.tex <==
\begin{table*}[t]
\footnotesize
\setlength{\tabcolsep}{3.3pt}
\renewcommand{\arraystretch}{1}
\centering
\caption{Evaluation Results for all variants of \tool across all SDCs. Best strategies are highlighted.}
\begin{tabular}{@{}lrrrrrrrrrrr@{\hskip 1.5em}rrrrrrrrr@{}}

\toprule

& \multicolumn{2}{c}{}
& \multicolumn{9}{c}{$\epsilon=0.05$, $1-\epsilon=0.95$}
& \multicolumn{9}{c}{$\epsilon=0.01$, $1-\epsilon=0.99$} \\

\cmidrule(r){4-12}
\cmidrule(r){13-21}

& \multicolumn{2}{c}{}
& \multicolumn{8}{c}{\it Unexpected}
& {Nominal}
& \multicolumn{8}{c}{\it Unexpected}
& {Nominal} \\

\cmidrule(r){4-11}
\cmidrule(r){12-12}
\cmidrule(r){13-20}
\cmidrule(r){21-21}

%& \multicolumn{10}{c}{\it Conditions}
%& {\it Conditions}
%& \multicolumn{8}{c}{\it Conditions}
%& {\it Conditions} \\

& \text{AUC-PRC$\boldsymbol{\uparrow}$}
& \text{AUC-ROC$\boldsymbol{\uparrow}$}
& \text{TP}
& \text{FP}
& \text{TN}
& \text{FN}
& \text{TPR$\boldsymbol{\uparrow}$}
& \text{FPR$\boldsymbol{\downarrow}$}
& \text{F1}
& \text{Prec.}
& \text{FPR$\boldsymbol{\downarrow}$}
& \text{TP}
& \text{FP}
& \text{TN}
& \text{FN}
& \text{TPR$\boldsymbol{\uparrow}$}
& \text{FPR$\boldsymbol{\downarrow}$}
& \text{F1}
& \text{Prec.}
& \text{FPR$\boldsymbol{\downarrow}$} \\

\midrule
\textit{\textbf{DAVE-2}}&       &       &     &     &        &     &       &       &        &        &       &     &     &        &     &       &       &       &       &       \\
\quad VAE                    & 0.354 & 0.902 & 149 & 304  & 1,970  & 47  & 0.760 & 0.134 & 0.459 & 0.329 & 0.042 & 107 & 183 & 2,959  & 89  & 0.546 & 0.058 & 0.440  & 0.369  & 0.003 \\
\quad DAE                    & 0.330 & 0.891 & 104 & 210  & 2,679  & 92  & 0.531 & 0.073 & 0.408 & 0.331 & 0.041 & 21  & 55  & 4,063  & 175 & 0.107 & 0.013 & 0.154  & 0.276  & 0.010 \\
\quad SAE                    & 0.336 & 0.891 & 138 & 260  & 1,877  & 58  & 0.704 & 0.122 & 0.465 & 0.347 & 0.050 & 108 & 183 & 2,665  & 88  & 0.551 & 0.064 & 0.444  & 0.371  & 0.002 \\
\quad CAE                    & 0.290 & 0.821 & 6   & 22   & 4,208  & 190 & 0.031 & 0.005 & 0.054 & 0.214 & 0.024 & 0   & 0   & 4,282  & 196 & 0 & 0 & n.a. & n.a. & 0 \\
\quad LSTM                   & 0.357 & 0.903 & 16  & 34   & 3,990  & 177 & 0.083 & 0.008 & 0.132 & 0.320 & 0 & 7   & 12  & 4,119  & 186 & 0.036 & 0.003 & 0.066  & 0.368  & 0 \\
\quad \deeproad              & 0.198 & 0.780 & 65  & 344  & 3,170  & 131 & 0.332 & 0.098 & 0.215 & 0.159 & 0.054 & 44  & 250 & 3,651  & 152 & 0.225 & 0.064 & 0.180  & 0.150  & 0.037 \\
\textit{\textbf{Epoch}}      &       &       &     &      &        &     &       &       &       &       &       &     &     &        &     &       &       &        &        &       \\
\quad VAE                    & 0.391 & 0.904 & 158 & 331  & 1,952  & 51  & 0.756 & 0.145 & 0.453 & 0.323 & 0.049 & 106 & 169 & 2,858  & 103 & 0.507 & 0.056 & 0.438  & 0.386  & 0.001 \\
\quad DAE                    & 0.399 & 0.895 & 112 & 188  & 2,720  & 97  & 0.536 & 0.065 & 0.440 & 0.373 & 0.042 & 24  & 34  & 3,653  & 185 & 0.115 & 0.009 & 0.180  & 0.414  & 0.010 \\
\quad SAE                    & 0.386 & 0.883 & 147 & 284  & 2,026  & 62  & 0.703 & 0.123 & 0.459 & 0.341 & 0.050 & 120 & 175 & 2,838  & 89  & 0.574 & 0.058 & 0.476  & 0.407  & 0.002 \\
\quad CAE                    & 0.310 & 0.822 & 6   & 23   & 3,661  & 203 & 0.029 & 0.006 & 0.050 & 0.207 & 0.020 & 0   & 0   & 3,731  & 209 & 0 & 0 & n.a. & n.a. & 0 \\
\quad LSTM                   & 0.385 & 0.879 & 23  & 34   & 3,503  & 175 & 0.116 & 0.010 & 0.180 & 0.404 & 0.001 & 7   & 13  & 3,592  & 191 & 0.035 & 0.004 & 0.064  & 0.350  & 0 \\
\quad \deeproad              & 0.213 & 0.807 & 70  & 308  & 2,917  & 139 & 0.335 & 0.096 & 0.239 & 0.185 & 0.053 & 43  & 201 & 3,240  & 166 & 0.206 & 0.058 & 0.190  & 0.176  & 0.040 \\
\textit{\textbf{Chauffeur}}  &       &       &     &      &        &     &       &       &       &       &       &     &     &        &     &       &       &        &        &       \\
\quad VAE                    & 0.242 & 0.951 & 98  & 392  & 3,700  & 23  & 0.810 & 0.096 & 0.321 & 0.200 & 0.049 & 81  & 267 & 5,391  & 40  & 0.669 & 0.047 & 0.345  & 0.233  & 0.002 \\
\quad DAE                    & 0.203 & 0.944 & 78  & 281  & 5,045  & 43  & 0.645 & 0.053 & 0.325 & 0.217 & 0.051 & 13  & 95  & 7,730  & 108 & 0.107 & 0.012 & 0.114  & 0.120  & 0.009 \\
\quad SAE                    & 0.241 & 0.931 & 96  & 354  & 3,650  & 25  & 0.793 & 0.088 & 0.336 & 0.213 & 0.056 & 86  & 240 & 5,177  & 35  & 0.711 & 0.044 & 0.385  & 0.264  & 0.003 \\
\quad CAE                    & 0.172 & 0.909 & 7   & 34   & 8,127  & 114 & 0.058 & 0.004 & 0.086 & 0.171 & 0.023 & 0   & 0   & 8,229  & 121 & 0 & 0 & n.a. & n.a. & 0 \\
\quad LSTM                   & 0.240 & 0.945 & 11  & 41   & 7,879  & 111 & 0.090 & 0.005 & 0.126 & 0.212 & 0 & 4   & 12  & 8,035  & 118 & 0.033 & 0.002 & 0.058  & 0.250  & 0 \\
\quad \deeproad              & 0.098 & 0.797 & 37  & 594  & 5,564  & 84  & 0.306 & 0.097 & 0.098 & 0.059 & 0.055 & 23  & 458 & 6,551  & 98  & 0.190 & 0.065 & 0.076  & 0.048  & 0.042 \\
\textit{\textbf{Totals}}     &       &       &     &      &        &     &       &       &       &       &       &     &     &        &     &       &       &        &        &       \\
\quad VAE                    & 0.320 & 0.924 & 405 & 1027 & 7,622  & 121 & 0.770 & 0.119 & 0.414 & 0.283 & 0.046 & 294 & 619 & 11,208 & 232 & 0.559 & 0.052 & 0.409  & 0.322  & 0.002 \\
\quad DAE                    & 0.301 & 0.911 & 294 & 679  & 10,444 & 232 & 0.559 & 0.061 & 0.392 & 0.302 & 0.045 & 58  & 184 & 15,446 & 468 & 0.110 & 0.012 & 0.151  & 0.240  & 0.009 \\
\quad SAE                    & 0.312 & 0.907 & 381 & 898  & 7,553  & 145 & 0.724 & 0.106 & 0.422 & 0.298 & 0.052 & 314 & 598 & 10,680 & 212 & 0.597 & 0.053 & 0.437  & 0.344  & 0.002 \\
\quad CAE                    & 0.255 & 0.864 & 19  & 79   & 15,996 & 507 & 0.036 & 0.005 & 0.061 & 0.194 & 0.022 & 0   & 0   & 16,242 & 526 & 0 & 0 & n.a. & n.a. & 0 \\
\quad LSTM                   & 0.329 & 0.915 & 50  & 109  & 15,372 & 463 & 0.098 & 0.007 & 0.149 & 0.315 & 0 & 18  & 37  & 15,746 & 495 & 0.035 & 0.002 & 0.063  & 0.327  & 0 \\
\quad \deeproad              & 0.159 & 0.799 & 172 & 1246 & 11,651 & 354 & 0.327 & 0.097 & 0.177 & 0.121 & 0.054 & 110 & 909 & 13,442 & 416 & 0.209 & 0.063 & 0.142  & 0.108  & 0.040 \\

\bottomrule

\end{tabular}
\label{tab:big_results_table}
\end{table*}


==> paper-anomaly-detection copy/table-results-99-999.tex <==
\begin{table*}[t]
\footnotesize
\setlength{\tabcolsep}{3.4pt}
\renewcommand{\arraystretch}{1}
\centering
\caption{Evaluation Results for all variants of \tool across all SDCs. Best strategies are highlighted.}
\begin{tabular}{@{}lrrrrrrrrrrr@{\hskip 1.5em}rrrrrrrrr@{}}

\toprule

& \multicolumn{2}{c}{}
& \multicolumn{9}{c}{\it Single image-based $\epsilon=0.99$}
& \multicolumn{9}{c}{\it Single image-based $\epsilon=0.999$} \\

\cmidrule(r){4-12}
\cmidrule(r){13-21}

& \multicolumn{2}{c}{}
& \multicolumn{8}{c}{\it Unexpected}
& {Nominal}
& \multicolumn{8}{c}{\it Unexpected}
& {Nominal} \\

\cmidrule(r){4-11}
\cmidrule(r){12-12}
\cmidrule(r){13-20}
\cmidrule(r){21-21}

%& \multicolumn{10}{c}{\it Conditions}
%& {\it Conditions}
%& \multicolumn{8}{c}{\it Conditions}
%& {\it Conditions} \\

& \text{AUC-PRC$\boldsymbol{\uparrow}$}
& \text{AUC-ROC$\boldsymbol{\uparrow}$}
& \text{TP}
& \text{FP}
& \text{TN}
& \text{FN}
& \text{TPR$\boldsymbol{\uparrow}$}
& \text{FPR$\boldsymbol{\downarrow}$}
& \text{F1}
& \text{Prec.}
& \text{FPR$\boldsymbol{\downarrow}$}
& \text{TP}
& \text{FP}
& \text{TN}
& \text{FN}
& \text{TPR$\boldsymbol{\uparrow}$}
& \text{FPR$\boldsymbol{\downarrow}$}
& \text{F1}
& \text{Prec.}
& \text{FPR$\boldsymbol{\downarrow}$} \\

\midrule

\textit{\textbf{DAVE-2}}             &       &       &     &     &        &     &       &       &        &        &       &     &     &        &     &       &       &       &       &       \\
\quad VAE      & 0.354 & 0.902 & 107 & 183 & 2,959  & 89  & 0.546 & 0.058 & 0.440 & 0.369 & 0.003 & 50  & 77  & 3,789  & 146 & 0.255 & 0.020 & 0.310 & 0.394 & 0     \\
\quad DAE     & 0.330 & 0.891 & 21  & 55  & 4,063  & 175 & 0.107 & 0.013 & 0.154 & 0.276 & 0.010 & 0   & 0   & 4,282  & 196 & 0 & 0 & n.a.  & n.a.  & 0     \\
\quad SAE     & 0.336 & 0.891 & 108 & 183 & 2,665  & 88  & 0.551 & 0.064 & 0.444 & 0.371 & 0.002 & 31  & 66  & 3,935  & 165 & 0.158 & 0.017 & 0.212 & 0.320 & 0     \\
\quad CAE     & 0.290 & 0.821 & 0   & 0   & 4,282  & 196 & 0 & 0 & n.a.  & n.a.  & 0 & 0   & 0   & 4,282  & 196 & 0 & 0 & n.a.  & n.a.  & 0     \\
\quad LSTM   & 0.357 & 0.903 & 7   & 12  & 4,119  & 186 & 0.036 & 0.003 & 0.066 & 0.368 & 0 & 1   & 4   & 4,143  & 192 & 0.005 & 0.001 & 0.010 & 0.200 & 0     \\
\quad \deeproad   & 0.198 & 0.780 & 44  & 250 & 3,651  & 152 & 0.225 & 0.064 & 0.180 & 0.150 & 0.037 & 23  & 127 & 3,985  & 173 & 0.117 & 0.031 & 0.133 & 0.153 & 0.034 \\ [0.5em]

\textit{\textbf{Epoch}}              &       &       &     &     &        &     &       &       &        &        &       &     &     &        &     &       &       &       &       &       \\
\quad VAE                & 0.391 & 0.904 & 106 & 169 & 2,858  & 103 & 0.507 & 0.056 & 0.438 & 0.385 & 0.001 & 49  & 60  & 3,352  & 160 & 0.234 & 0.018 & 0.308 & 0.450 & 0 \\
\quad DAE                & 0.399 & 0.895 & 24  & 34  & 3,653  & 185 & 0.115 & 0.009 & 0.180 & 0.414 & 0.010 & 0   & 0   & 3,731  & 209 & 0 & 0 & n.a.  & n.a.  & 0 \\
\quad SAE                & 0.386 & 0.883 & 120 & 175 & 2,838  & 89  & 0.574 & 0.058 & 0.476 & 0.407 & 0.002 & 26  & 51  & 3,523  & 183 & 0.124 & 0.014 & 0.182 & 0.338 & 0 \\
\quad CAE                & 0.310 & 0.822 & 0   & 0   & 3,731  & 209 & 0 & 0 & n.a.   & n.a.   & 0 & 0   & 0   & 3,731  & 209 & 0 & 0 & n.a.  & n.a.  & 0 \\
\quad LSTM               & 0.385 & 0.879 & 7   & 13  & 3,592  & 191 & 0.035 & 0.004 & 0.064 & 0.350 & 0 & 0   & 4   & 3,621  & 198 & 0 & 0.001 & n.a.  & 0 & 0 \\
\quad \deeproad           & 0.213 & 0.807 & 43  & 201 & 3,240  & 166 & 0.206 & 0.058 & 0.190 & 0.176 & 0.040 & 23  & 118 & 3,512  & 186 & 0.110 & 0.033 & 0.131 & 0.163 & 0.027 \\ [0.5em]

\textit{\textbf{Chauffeur}}  &       &       &     &     &        &     &       &       &        &        &       &     &     &        &     &       &       &       &       &       \\
\quad VAE                & 0.242 & 0.951 & 81  & 267 & 5,391  & 40  & 0.669 & 0.047 & 0.345 & 0.233 & 0.002 & 50  & 100 & 7,070  & 71  & 0.413 & 0.014 & 0.369 & 0.333 & 0 \\
\quad DAE                & 0.203 & 0.944 & 13  & 95  & 7,730  & 108 & 0.107 & 0.012 & 0.114 & 0.120 & 0.009 & 0   & 1   & 8,228  & 121 & 0 & 0 & n.a.  & 0 & 0 \\
\quad SAE                & 0.241 & 0.931 & 86  & 240 & 5,177  & 35  & 0.711 & 0.044 & 0.385 & 0.264 & 0.003 & 34  & 104 & 7,483  & 87  & 0.281 & 0.014 & 0.263 & 0.246 & 0 \\
\quad CAE                & 0.172 & 0.909 & 0   & 0   & 8,229  & 121 & 0 & 0 & n.a.   & n.a.   & 0 & 0   & 0   & 8,229  & 121 & 0 & 0 & n.a.  & n.a.  & 0 \\
\quad LSTM               & 0.240 & 0.945 & 4   & 12  & 8,035  & 118 & 0.033 & 0.002 & 0.058 & 0.250 & 0 & 0   & 2   & 8,079  & 122 & 0 & 0 & n.a.  & 0 & 0 \\
\quad \deeproad           & 0.098 & 0.797 & 23  & 458 & 6,551  & 98  & 0.190 & 0.065 & 0.076 & 0.048 & 0.042 & 14  & 264 & 7,419  & 107 & 0.116 & 0.034 & 0.070 & 0.050 & 0.035 \\ [0.5em]

\textit{\textbf{Totals}} &       &       &     &     &        &     &       &       &        &        &       &     &     &        &     &       &       &       &       &       \\
\quad VAE                & 0.320 & 0.924 & 294 & 619 & 11,208 & 232 & 0.559 & 0.052 & 0.409 & 0.322 & 0.002 & 149 & 237 & 14,211 & 377 & 0.283 & 0.016 & 0.327 & 0.386 & 0 \\
\quad DAE                & 0.301 & 0.911 & 58  & 184 & 15,446 & 468 & 0.110 & 0.012 & 0.151 & 0.240 & 0.009 & 0   & 1   & 16,241 & 526 & 0 & 0 & n.a.  & 0 & 0 \\
\quad SAE                & 0.312 & 0.907 & 314 & 598 & 10,680 & 212 & 0.597 & 0.053 & 0.437 & 0.344 & 0.002 & 91  & 221 & 14,941 & 435 & 0.173 & 0.015 & 0.217 & 0.292 & 0 \\
\quad CAE                & 0.255 & 0.864 & 0   & 0   & 16,242 & 526 & 0 & 0 & n.a.   & n.a.   & 0 & 0   & 0   & 16,242 & 526 & 0 & 0 & n.a.  & n.a.  & 0 \\
\quad LSTM               & 0.329 & 0.915 & 18  & 37  & 15,746 & 495 & 0.035 & 0.002 & 0.064 & 0.327 & 0 & 1   & 10  & 15,843 & 512 & 0.002 & 0.001 & 0.004 & 0.091 & 0 \\
\quad \deeproad           & 0.159 & 0.799 & 110 & 909 & 13,442 & 416 & 0.209 & 0.063 & 0.142 & 0.108 & 0.040 & 60  & 509 & 14,916 & 466 & 0.114 & 0.033 & 0.110 & 0.105 & 0.032 \\

\bottomrule

\end{tabular}
\label{tab:big_results_table}
\end{table*}


==> table-results-99-999.tex <==
\begin{table*}[t]
\footnotesize
\setlength{\tabcolsep}{3.4pt}
\renewcommand{\arraystretch}{1}
\centering
\caption{Evaluation Results for all variants of \tool across all SDCs. Best strategies are highlighted.}
\begin{tabular}{@{}lrrrrrrrrrrr@{\hskip 1.5em}rrrrrrrrr@{}}

\toprule

& \multicolumn{2}{c}{}
& \multicolumn{9}{c}{\it Single image-based $\epsilon=0.99$}
& \multicolumn{9}{c}{\it Single image-based $\epsilon=0.999$} \\

\cmidrule(r){4-12}
\cmidrule(r){13-21}

& \multicolumn{2}{c}{}
& \multicolumn{8}{c}{\it Unexpected}
& {Nominal}
& \multicolumn{8}{c}{\it Unexpected}
& {Nominal} \\

\cmidrule(r){4-11}
\cmidrule(r){12-12}
\cmidrule(r){13-20}
\cmidrule(r){21-21}

%& \multicolumn{10}{c}{\it Conditions}
%& {\it Conditions}
%& \multicolumn{8}{c}{\it Conditions}
%& {\it Conditions} \\

& \text{AUC-PRC$\boldsymbol{\uparrow}$}
& \text{AUC-ROC$\boldsymbol{\uparrow}$}
& \text{TP}
& \text{FP}
& \text{TN}
& \text{FN}
& \text{TPR$\boldsymbol{\uparrow}$}
& \text{FPR$\boldsymbol{\downarrow}$}
& \text{F1}
& \text{Prec.}
& \text{FPR$\boldsymbol{\downarrow}$}
& \text{TP}
& \text{FP}
& \text{TN}
& \text{FN}
& \text{TPR$\boldsymbol{\uparrow}$}
& \text{FPR$\boldsymbol{\downarrow}$}
& \text{F1}
& \text{Prec.}
& \text{FPR$\boldsymbol{\downarrow}$} \\

\midrule

\textit{\textbf{DAVE-2}}             &       &       &     &     &        &     &       &       &        &        &       &     &     &        &     &       &       &       &       &       \\
\quad VAE      & 0.354 & 0.902 & 107 & 183 & 2,959  & 89  & 0.546 & 0.058 & 0.440 & 0.369 & 0.003 & 50  & 77  & 3,789  & 146 & 0.255 & 0.020 & 0.310 & 0.394 & 0     \\
\quad DAE     & 0.330 & 0.891 & 21  & 55  & 4,063  & 175 & 0.107 & 0.013 & 0.154 & 0.276 & 0.010 & 0   & 0   & 4,282  & 196 & 0 & 0 & n.a.  & n.a.  & 0     \\
\quad SAE     & 0.336 & 0.891 & 108 & 183 & 2,665  & 88  & 0.551 & 0.064 & 0.444 & 0.371 & 0.002 & 31  & 66  & 3,935  & 165 & 0.158 & 0.017 & 0.212 & 0.320 & 0     \\
\quad CAE     & 0.290 & 0.821 & 0   & 0   & 4,282  & 196 & 0 & 0 & n.a.  & n.a.  & 0 & 0   & 0   & 4,282  & 196 & 0 & 0 & n.a.  & n.a.  & 0     \\
\quad LSTM   & 0.357 & 0.903 & 7   & 12  & 4,119  & 186 & 0.036 & 0.003 & 0.066 & 0.368 & 0 & 1   & 4   & 4,143  & 192 & 0.005 & 0.001 & 0.010 & 0.200 & 0     \\
\quad \deeproad   & 0.198 & 0.780 & 44  & 250 & 3,651  & 152 & 0.225 & 0.064 & 0.180 & 0.150 & 0.037 & 23  & 127 & 3,985  & 173 & 0.117 & 0.031 & 0.133 & 0.153 & 0.034 \\ [0.5em]

\textit{\textbf{Epoch}}              &       &       &     &     &        &     &       &       &        &        &       &     &     &        &     &       &       &       &       &       \\
\quad VAE                & 0.391 & 0.904 & 106 & 169 & 2,858  & 103 & 0.507 & 0.056 & 0.438 & 0.385 & 0.001 & 49  & 60  & 3,352  & 160 & 0.234 & 0.018 & 0.308 & 0.450 & 0 \\
\quad DAE                & 0.399 & 0.895 & 24  & 34  & 3,653  & 185 & 0.115 & 0.009 & 0.180 & 0.414 & 0.010 & 0   & 0   & 3,731  & 209 & 0 & 0 & n.a.  & n.a.  & 0 \\
\quad SAE                & 0.386 & 0.883 & 120 & 175 & 2,838  & 89  & 0.574 & 0.058 & 0.476 & 0.407 & 0.002 & 26  & 51  & 3,523  & 183 & 0.124 & 0.014 & 0.182 & 0.338 & 0 \\
\quad CAE                & 0.310 & 0.822 & 0   & 0   & 3,731  & 209 & 0 & 0 & n.a.   & n.a.   & 0 & 0   & 0   & 3,731  & 209 & 0 & 0 & n.a.  & n.a.  & 0 \\
\quad LSTM               & 0.385 & 0.879 & 7   & 13  & 3,592  & 191 & 0.035 & 0.004 & 0.064 & 0.350 & 0 & 0   & 4   & 3,621  & 198 & 0 & 0.001 & n.a.  & 0 & 0 \\
\quad \deeproad           & 0.213 & 0.807 & 43  & 201 & 3,240  & 166 & 0.206 & 0.058 & 0.190 & 0.176 & 0.040 & 23  & 118 & 3,512  & 186 & 0.110 & 0.033 & 0.131 & 0.163 & 0.027 \\ [0.5em]

\textit{\textbf{Chauffeur}}  &       &       &     &     &        &     &       &       &        &        &       &     &     &        &     &       &       &       &       &       \\
\quad VAE                & 0.242 & 0.951 & 81  & 267 & 5,391  & 40  & 0.669 & 0.047 & 0.345 & 0.233 & 0.002 & 50  & 100 & 7,070  & 71  & 0.413 & 0.014 & 0.369 & 0.333 & 0 \\
\quad DAE                & 0.203 & 0.944 & 13  & 95  & 7,730  & 108 & 0.107 & 0.012 & 0.114 & 0.120 & 0.009 & 0   & 1   & 8,228  & 121 & 0 & 0 & n.a.  & 0 & 0 \\
\quad SAE                & 0.241 & 0.931 & 86  & 240 & 5,177  & 35  & 0.711 & 0.044 & 0.385 & 0.264 & 0.003 & 34  & 104 & 7,483  & 87  & 0.281 & 0.014 & 0.263 & 0.246 & 0 \\
\quad CAE                & 0.172 & 0.909 & 0   & 0   & 8,229  & 121 & 0 & 0 & n.a.   & n.a.   & 0 & 0   & 0   & 8,229  & 121 & 0 & 0 & n.a.  & n.a.  & 0 \\
\quad LSTM               & 0.240 & 0.945 & 4   & 12  & 8,035  & 118 & 0.033 & 0.002 & 0.058 & 0.250 & 0 & 0   & 2   & 8,079  & 122 & 0 & 0 & n.a.  & 0 & 0 \\
\quad \deeproad           & 0.098 & 0.797 & 23  & 458 & 6,551  & 98  & 0.190 & 0.065 & 0.076 & 0.048 & 0.042 & 14  & 264 & 7,419  & 107 & 0.116 & 0.034 & 0.070 & 0.050 & 0.035 \\ [0.5em]

\textit{\textbf{Totals}} &       &       &     &     &        &     &       &       &        &        &       &     &     &        &     &       &       &       &       &       \\
\quad VAE                & 0.320 & 0.924 & 294 & 619 & 11,208 & 232 & 0.559 & 0.052 & 0.409 & 0.322 & 0.002 & 149 & 237 & 14,211 & 377 & 0.283 & 0.016 & 0.327 & 0.386 & 0 \\
\quad DAE                & 0.301 & 0.911 & 58  & 184 & 15,446 & 468 & 0.110 & 0.012 & 0.151 & 0.240 & 0.009 & 0   & 1   & 16,241 & 526 & 0 & 0 & n.a.  & 0 & 0 \\
\quad SAE                & 0.312 & 0.907 & 314 & 598 & 10,680 & 212 & 0.597 & 0.053 & 0.437 & 0.344 & 0.002 & 91  & 221 & 14,941 & 435 & 0.173 & 0.015 & 0.217 & 0.292 & 0 \\
\quad CAE                & 0.255 & 0.864 & 0   & 0   & 16,242 & 526 & 0 & 0 & n.a.   & n.a.   & 0 & 0   & 0   & 16,242 & 526 & 0 & 0 & n.a.  & n.a.  & 0 \\
\quad LSTM               & 0.329 & 0.915 & 18  & 37  & 15,746 & 495 & 0.035 & 0.002 & 0.064 & 0.327 & 0 & 1   & 10  & 15,843 & 512 & 0.002 & 0.001 & 0.004 & 0.091 & 0 \\
\quad \deeproad           & 0.159 & 0.799 & 110 & 909 & 13,442 & 416 & 0.209 & 0.063 & 0.142 & 0.108 & 0.040 & 60  & 509 & 14,916 & 466 & 0.114 & 0.033 & 0.110 & 0.105 & 0.032 \\

\bottomrule

\end{tabular}
\label{tab:big_results_table}
\end{table*}

